Classifier-independent Lower-Bounds for Adversarial Robustness

We theoretically analyse the limits of robustness to test-time adversarial and noisy examples in classification. Our work focuses on deriving bounds which uniformly apply to all classifiers (i.e all measurable functions from features to labels) for a given problem. Our contributions are two-fold. (1) We use optimal transport theory to derive variational formulae for the Bayes-optimal error a classifier can make on a given classification problem, subject to adversarial attacks. The optimal adversarial attack is then an optimal transport plan for a certain binary cost-function induced by the specific attack model, and can be computed via a simple algorithm based on maximal matching on bipartite graphs. (2) We derive explicit lower-bounds on the Bayes-optimal error in the case of the popular distance-based attacks. These bounds are universal in the sense that they depend on the geometry of the class-conditional distributions of the data, but not on a particular classifier. Our results are in sharp contrast with the existing literature, wherein adversarial vulnerability of classifiers is derived as a consequence of nonzero ordinary test error.

==> 011-notations-table.tex <==
\begin{table*}[!h]  
   \centering
 \begin{tabular}{|c|c|}
 \hline
   Notation & Meaning\\
   \hline
   \hline
   $\mathcal X$ & Feature space, typically a separable Banach space (like $\mathbb R^d$ equipped with an $\ell_p$-norm),\\
   & or more generally a Polish space\\\hline
  
   $\mathcal A$, $a$ & An adversarial adversarial attack model on $\mathcal X$, i.e a prescribtion of a neighborhood\\
   & $\mathcal A_x$ for each $x \in \mathcal X$. A type-$\mathcal A$ attack is a measurable map $a:\mathcal X \times \{\pm 1\} \rightarrow \mathcal X$\\
   & such that $a(x,y) \in \mathcal A_x$ for all $(x,y) \in \mathcal X \times \{\pm 1\}$ \\ \hline
  $P_{\pm}$ & Except otherwise stated, these are class-conditional distributions of the covariates $X$.\\
  &$\diff P^+(x) = \diff P(X=x,Y=+1)$, $\diff P^-(x) = \diff P(X=x,Y=-1)$\\\hline
   $a_{\pm}$ & Given a type-$\mathcal A$ attack $a:\mathcal X \times \{\pm 1\} \rightarrow \mathcal X$, define
            $a_y(x):=a(x,y)\;\forall (x,y)\in \mathcal X \times \{\pm 1\}$\\\hline
 $\err_{\mathcal A}(h)$ & Classification error of a classifier $h$ against type-$\mathcal A$ adversarial attacks \\ \hline
 $\err_{\mathcal A}^*$ & Least possible classification error of a classifier against type-$\mathcal A$ adversarial attacks \\ \hline
 $\ot_{\mathcal A}$ & Optimal-transport metric generated by adversarial attack model $\mathcal A$; defined in eqn. \eqref{eq:otdef} \\ \hline
 $\tv_{\mathcal A}$ & Total-variation metric generated by adversarial attack model $\mathcal A$; defined in Theorem \ref{thm:badass}\\ \hline
 \end{tabular}
 \caption{Summary of key notations used in manuscript.}
 \label{Tab:notations}
 \end{table*}
 
 \todo{Define total-variation!}

==> 03-experiments.tex <==
\section{Experimental results}
% ...

==> awgn.tex <==
\begin{wrapfigure}{r}{0.32\textwidth}
  \vspace{-.6cm}
  \centering
  \begin{tikzpicture}[scale=1.8, thick]
% arrows
\draw [->, line width = 0.4mm] (0.1,0) -- (0.5,0);
\draw [->, line width = 0.4mm] (.9,0) -- (1.3,0);
\draw [->, line width = 0.4mm] (1.7,0) -- (2.1,0);
\draw [->, line width = 0.4mm] (.7,-0.7) -- (.7,-0.2);

% circle
\draw (.7,-0.15) -- (.7,0.15);
\draw (.85,0) -- (0.55,0);

% plus sign
\draw[fill=red,opacity=.4] (.7,0) circle [radius = .2];

% text
\node at (-0.02, 0) {\large $x$};
% \node at (2.1, 0) {\large $x'$};
\node at (1.5,0) [rectangle,fill=cyan,scale=3.4] (toto) {};
\node at (1.5, 0) {\large $h$};
\node at (2.2, 0) {\large $\hat{y}$};
\node at (.7, -0.8) {\large $\mathcal{N}(0,\varepsilon^2 I)$};
\end{tikzpicture}
\vspace{-.7cm}
\caption{Classification in a Hilbert space $\mathcal X$ under corruption by
  isotropic Gaussian noise % . Here the Markov kernel is given by
  $\omega_x = x +
  \mathcal N(0,\varepsilon^2 I),\;\forall x \in \mathcal X$.
  % Here $h:\mathcal X \rightarrow \{1,2\}$ is the classifier (e.g a deep neural net).
}
\label{fig:awgn}
\end{wrapfigure}


==> bridge.tex <==
\section{From noise to adversaries: bounds from spectral analysis}
Let $h:\mathcal X \rightarrow \mathcal Z$ be a measurable function between {\bfseries finite-dimensional} normed vector-spaces. For example, this could be the representation layers of a deep neural network, in which case $\mathcal X$ would be the input space of a deep neural network, and $\mathcal Z$ would be the output of the logit layer (i.e penultimate layer before prediction).

\subsection{Preliminaries}
\begin{restatable}[Worst-case and average-case directional rates of change]{df}{} For $x \in \mathcal X$, define the worst possible directional rate of change of $h$ at $x$, denoted $\Delta_{\max} h(x)$ by
$$
\Delta_{\max} h(x) := \liminf_{\epsilon \rightarrow 0^+} h_{\max}^\epsilon(x), \text{ with }\Delta_{\max}^\epsilon h(x) := \sup_{\|\delta x\|_{\mathcal X} \le 1}\frac{\|h(x+\epsilon \delta x) - h(x)\|_{\mathcal Z}}{\epsilon}.
$$
Also define the average fluctuation of $h$ at $x$ as
$$
\overline{\Delta} h(x) := \limsup_{\epsilon \rightarrow 0^+}\overline{\Delta}^\epsilon h(x), \text{ with }
\overline{\Delta}^\epsilon h(x) := \frac{\mathbb E_u\|h(x + \epsilon u) - h(x)\|_{\mathcal Z}}{\epsilon},
$$
where $u$ is uniformly distributed on the unit ball of $\mathcal X$.
\end{restatable}

\begin{restatable}[Fr\'echet differentiability]{df}{}
$h$ is said to be (Fr\'echet) differentiable at $x$ it there exists a continuous linear operator $\nabla f(x)$, called the Fr\'echet derivative of $h$ at $x$, such that the following first-order approximation is valid
\begin{eqnarray}
\|h(x+\delta x)-h(x) - \epsilon \nabla h(x)\delta x\|_{\mathcal Z} = o(\epsilon),\text{ for every }\epsilon > 0\text{ and }\delta x \in \mathbb S_{\mathcal X},
\label{eq:frechet}
\end{eqnarray}
where $\lim_{\epsilon \rightarrow 0^+}o(\epsilon)/\epsilon = 0$.
\end{restatable}

\begin{restatable}{lm}{}
If the function $h:\mathcal X \rightarrow \mathcal Z$ is differentiable at $x$, then $\Delta_{\max} h(x) = \|\nabla h(x)\|_{\mathcal X,\mathcal Z}$ and $\overline{\Delta h}(x) = \nabla_{\mathcal X,\mathcal Z}(\nabla h(x))$.
\label{lm:diffble}
\end{restatable}  
\begin{proof}
Since, $h$ is (Fr\'echet) differentiable at $x$, the approximation \eqref{eq:frechet} holds, from which we easily obtain that $\|h(x+\delta x)-h(x)\|_{\mathcal Z} = \epsilon\|\nabla h(x)\delta x\| + o(\epsilon)$.
Thus,
\begin{eqnarray*}
\begin{split}
\overline{\Delta} h(x) &:= \liminf_{\epsilon \rightarrow 0^+}\sup_{\|\delta x\|_{\mathcal X} \le 1}\frac{\|h(x+\epsilon\delta x) - h(x)\|_{\mathcal Z}}{\epsilon} = \liminf_{\epsilon \rightarrow 0^+}\sup_{\|\delta x\| \le 1}\|\nabla h(x)\delta x\|_{\mathcal Z} + o(\epsilon)/\epsilon\\
&=\sup_{\|\delta x\| \le 1}\liminf_{\epsilon \rightarrow 0^+}\|\nabla h(x)\delta x\|_{\mathcal Z} + o(\epsilon)/\epsilon = \sup_{\|\delta x\|_{\mathcal X} \le 1}\|\nabla h(x)\delta x\|_{\mathcal Z} =: \|\nabla h(x)\|_{\mathcal X,\mathcal Z}.
\end{split}
\end{eqnarray*}

On the other hand, if $u$ is uniformly random on the sphere $\mathbb S_{\mathcal X} := \{x \in \mathcal X \mid \|x\|_{\mathcal X} = 1\}$.

\begin{eqnarray*}
\begin{split}
\overline{\Delta} h(x) &:= \frac{\lim_{\epsilon \rightarrow 0}\mathbb E_u\|h(x+\epsilon u) - h(x)\|_{\mathcal Z}}{\epsilon} = \lim_{\epsilon \rightarrow 0^+}\mathbb E_u\|\nabla h(x)u\|_{\mathcal Z} + o(\epsilon)/\epsilon = \mathbb E_u\|\nabla h(x)u\|_{\mathcal Z}\\
&= \Delta_{\mathcal X,\mathcal Z}(\nabla h(x)).
\end{split}
\end{eqnarray*}
\end{proof}

\begin{restatable}[Operator norm]{df}{}
Given a linear operator (i.e a matrix) $A: \mathcal X \rightarrow \mathcal Z$, its operator norm denoted $\|A\|_{\mathcal X,\mathcal Z}$, is the largest distortion $A$ can cause to the norm of an input vector, or more precisely
\begin{eqnarray}
\|A\|_{\mathcal X,\mathcal Z} := \sup_{\|x\|_{\mathcal X} \le 1}\|Ax\|_{\mathcal Z}=\sup_{x \in \mathcal X,\;x \ne 0}\frac{\|Ax\|_{\mathcal Z}}{\|x\|_{\mathcal X}}.
\label{eq:pqnorm}
\end{eqnarray}
\label{df:pqnorm}
\end{restatable}

Since there can be different norms on the same underlying vector-space, we say that the operator norm $\|\cdot\|_{\mathcal X,\mathcal Z}$ is \emph{induced} by the norms $\|\cdot\|_{\mathcal X}$ and $\|\cdot\|_{\mathcal Z}$ prescribed on the vector-spaces $\mathcal X$ and $\mathcal Z$. For example if $\mathcal X$ and $\mathcal Z$ are finite-dimensional euclidean spaces (i.e some $\mathbb R^m$ and $\mathbb R^k$ equipped with the $\ell_2$ induced by the dot product), then $\|A\|_{\mathcal X,\mathcal Z}$ is precisely the spectral norm of $A$, i.e, its largest singular-value, usually denoted $\|A\|_2$. In the one-dimensional output case where $\mathcal Z = (\mathbb R,|\cdot|)$, $A$ is just a linear functional and $\|A\|_{\mathcal X,\mathcal Z} = \|A\|_{\mathcal X^*}$.\\

Our interest linear operators is not artifical. They will be the building-block of our later analysis of adversarial attacks for linear models (e.g logistic regression) and nonlinear models (e.g deep neural networks) alike.

\begin{restatable}[Singular-values, rank, spectral norm, Frobenius norm]{df}{}
Given a matrix $A \in \mathbb R^{k \times m}$ (i.e linear operator $A:\mathbb R^m \rightarrow \mathbb R^k$), its singular-values
$$
\sigma_1(A) \ge  \sigma_2(A) \ge \ldots \ge \sigma_r(A) > \sigma_{r+1}(A) = \ldots \sigma_{\min(m,k)} = 0
$$
are positive square-roots of the eigenvalues of the positive semi-definite matrix $A^TA$. The number of nonzero singular-values $r$ is called the rank  of $A$, denoted $\rank A$. The Frobenius norm of $A$, denoted $\|A\|_F$, is $\ell_2$-norm of the vector of singular-values, i.e $\|A\|_F := (\sum_{j=1}^{\rank A}\sigma_j(A)^2)^{1/2}$.
\end{restatable}
% \begin{restatable}[Shartten $p$-norms]{df}{}
% Let $\sigma_1 \ge \sigma_2 \ldots \ldots \sigma_r > 0$ be the nonzero singular-values of $A$ (so that $\rank(A) = r$) collected in to vector $\sigma \in \mathbb R^r$, and let $p \in [1,p]$. The Shatten $p$-norm of $A$
% \end{restatable}
\begin{restatable}{lm}{}
$\|A\|_2 = \sigma_1(A)$.
\end{restatable}
For this reason, the matrix-norm $\|A\|_2$ induced by the euclidean norm on its domain vector-space $\mathbb R^m$ and co-domain vector-space $\mathbb R^n$ is also called the spectral norm of $A$.

\begin{restatable}[Comparison between spectral and Frobenius norms]{lm}{}
$\sigma_1(A) \le \|A\|_F \le \sigma_1(A)\sqrt{\rank A}$.
\label{lm:specvsfro}
\end{restatable}

\subsection{Average norm-distortion (AND) coefficient of a matrix}
We now consider linear operators between normed vector-spaces. Given $p \in [1, \infty]$ and $x \in \mathbb R^m$, recall that the $\ell_p$-norm of $x$ is defined by
$$
\|x\|_p := \begin{cases}(\sum_{j=1}^m|x_j|^p)^{1/p},&\mbox{ if }1 \le p < \infty,\\\max_{j=1}^m|x_j|,&\mbox{ if }p=\infty.\end{cases}
$$

% \begin{restatable}{df}{}
For $p,q \in [1,\infty]$, define
\begin{eqnarray}
\theta_{p,q} := (1/p-1/q)_+,
\label{eq:thetapq}
\end{eqnarray}
which (as we see in the well-known lemma below) controls how distorted the $\ell_p$ and $\ell_q$ norms are from one another.
% \end{restatable}

Note that for all $p,q \in [1,\infty]$, it holds that
\begin{itemize}
    \item $\theta_{p,q} \ge 0$, with equality iff $p \ge q$.
    \item $\theta_{p,1} = \theta_{\infty,p} = 1$.
    \item $\min(\theta_{p,q},\theta_{q,p})=0$.
    \item $\theta_{p,q} + \theta_{q,p} = \max(\theta_{p,q},\theta_{q,p}) =  |1/p-1/q| \le 1$.
    \item $\theta_{p,q} - \theta_{q,p} = 1/p-1/q \in [-1, 1]$.
\end{itemize}

\begin{restatable}[Equivalence of norms in finite-dimensions]{lm}{}
Let $p,q \in [1,\infty]$ and $x \in \mathbb R^d$. It holds that
\begin{eqnarray}
d^{\theta_{p,q}}\|x\|_p \le \|x\|_q \le d^{\theta_{q,p}}\|x\|_p.
\end{eqnarray}
\label{lm:lpequiv}
\end{restatable}
\begin{proof}
Classic. Uses Hoelder's inequality.
\end{proof}
The above Lemma can be used to proof Lemma \ref{lm:specvsfro}, since by definition, $\sigma_1(A)$ is the $\ell_\infty$ norm of the vector of singular-values, and $\|A\|_F$ is their $\ell_2$-norm.

\subsubsection{Geoemtry of the unit sphere in $\ell_p^m$} The normed vector-space $(\mathbb R^m,\ell_p)$ will be abbreviated $\ell_p^m$.
The unit-sphere in $\ell_p^m$ will be denoted $\mathbb S_p^m$. Formally, 
\begin{eqnarray}
\mathbb S_p^m := \{x \in \mathbb R^m \mid \|x\|_p = 1\}.
\end{eqnarray}

\begin{restatable}[AND: Average norm-distortion coefficient of a matrix]{df}{}
Let $u$ be uniformly distributed on $\mathbb S_p^m$, and define the average norm-distortion (AND) coefficient of $A$ is the quantity $\Delta_{p,q}(A):= \mathbb E_u\|Au\|_q$.
\end{restatable}

{\bfseries Question.} \textit{What are good upper bounds for the average norm-distortion coefficient $\Delta_{p,q}(A)$ in terms of spectral properties of $A$ ($m$, $k$, singular-values, etc.) ?
}\\

To warm up, lets begin by answering the above question in the euclidean case $p=q=2$.

\begin{restatable}[Upper bound on the AND coefficient in euclidean setting]{lm}{}
It holds that $\Delta_{2,2}(A) \le m^{-1/2}\|A\|_{F}$.
\end{restatable}
\begin{proof}
In this case $z$ is uniform on the euclidean unit $m$-sphere, and so has mean $\mu = 0$ and covariance matrix $\Sigma = (1/m)I_m$. By Jensen's inequality and standard formulae for expectation of quadratic forms], one computes
\begin{eqnarray*}
\begin{split}
\Delta_{2,2}(A)^2 &:= (\mathbb E_u\|Au\|_2)^2 \le \mathbb E_u\|Au\|_2^2 = \trace(A^TA\Sigma) + \|A\mu\|_2^2 = (1/m)\trace(A^TA)
= (1/m)\|A\|_{F}^2,
\end{split}
\end{eqnarray*}

from which we get $\Delta_{2,2}(A) \le m^{-1/2}\|A\|_{F}$.
\end{proof}

The next Lemma shows that the covariance matrix of the uniform random vector on the $\mathbb S_p^m$ has coordinates with individual variance $\mathcal O(m^{-2/p})$ for large $m$, and zero cross-variance.
\begin{restatable}[Mean and covariance matrix of the uniform random variable in $\mathbb S_p^m$]{lm}{lpcov}
Let $u$ be uniformly distributed on unit sphere $\mathbb S_p^m$. Let $\Gamma: (0, \infty) \rightarrow [0,\infty)$ be the so-called \emph{gamma function} defined by $\Gamma(a) := \int_0^\infty t^{a-1}e^{-t}dt$. Then, $u$ has zero mean and covariance matrix $\Sigma_{m,p} = \sigma_{m,p}^2I_m$, where
$$
\sigma_{m,p}^2 := \dfrac{p^{-2/p}\Gamma(3/p)}{\Gamma(1/p)}m^{-2/p} \le \begin{cases} 2m^{-2/p},&\mbox{ if }1 \le p < 2,\\
m^{-2/p},&\mbox{ if }2 \le p < \infty,\\
1/3,&\mbox{ if }p = \infty,\end{cases}
$$
with equality if $p \in \{1,2,\infty\}$.
\label{lm:lpcov}
\end{restatable}

\begin{proof}
By symmetry, $u$ has zero mean indeed. Also, it is clear that the covariance matrix $\Sigma$ is diagonal. This is because for every sign vector $s \in \{\pm 1\}^m$, $(s_1u_1,\ldots,s_mu_m)$ has the same distribution as $u$; thus $\mathbb E[u_iu_j] = -\mathbb E[u_iu_j]$ whenever $i \ne j$, and so the off-diagonal entries of $\Sigma$ are $\mathbb E[u_iu_j] = 0$. Also, by symmetry, the coordinates of $u$ are identically distributed. Thus, $\Sigma_{m,p} = \sigma_{m,p}^2I_m$, where $\sigma_{m,p}^2 := \var(u_1)> 0$. It then remains to compute $\sigma_{m, p}^2$.\\

Let $p \in [1,\infty)$ and $b := (m-1)/p \in (0, \infty)$. By Theorem 2.1 of ~\cite{lpsphere}, the marginal density of $u_1$ is $t \mapsto \dfrac{p\Gamma(m/p)}{2\Gamma(1/p)\Gamma(b)}(1-|t|^p)^{b - 1}\mathbbm{1}_{[-1, 1]}(t)$.
Thus, the variance of $u_1$ writes
$$
\sigma_{m,p}^2 = \mathbb Eu_1^2 - (\mathbb E u_1)^2 = \mathbb Eu_1^2 =  \dfrac{p\Gamma(m/p)}{2\Gamma(1/p)\Gamma((m-1)/p)}(1-|t|^p)^{b - 1} I_{m,p},
$$
where $I_{m,p} := \int_{-1}^1t^2(1-|t|^p)^{b- 1}dt = 2\int_0^1 t^2(1-t^p)^{b-1} dt$. Now, for $t \in [0, 1]$, consider the change of variable $t^p = s$, so that $s \in [0, 1]$, $t = s^{1/p}$ and $t^2dt = s^{2/p}\cdot 1/p \cdot s^{1/p-1}ds=(1/p)s^{3/p-1}ds$. Then, we can rewrite
$$
I_{m,p} = (2/p)\int_0^{1}s^{3/p-1}(1-s)^{b-1}ds = (2/p)B(3/p,b).
$$
where $B(a,b) := \dfrac{\Gamma(a)\Gamma(b)}{\Gamma(a+b)}$ is the \emph{beta function}. 
Substituting $b = (m-1) / p$, we then obtain
$$
I_{m,p} = (2/p)B(3/p,(m-1)/p) = \dfrac{(2/p)\Gamma(3/p)\Gamma((m-1)/p)}{\Gamma((m+2)/p)}.
$$
Therefore, putting things together yields
\begin{eqnarray*}
\begin{split}
\sigma_{m,p}^2 &= \dfrac{p\Gamma(m/p)}{2\Gamma(1/p)\Gamma((m-1)/p)}I_{m,p} = \dfrac{p\Gamma(m/p)}{2\Gamma(1/p)\Gamma((m-1)/p)}\dfrac{(2/p)\Gamma(3/p)\Gamma((m-1)/p)}{\Gamma((m+2)/p)}\\
&= \dfrac{\Gamma(m/p)\Gamma(3/p)}{\Gamma(1/p)\Gamma((m+2)/p)}\approx \dfrac{\Gamma(m/p)\Gamma(3/p)}{\Gamma(1/p)\Gamma(m/p)(m/p)^{2/p}} = \frac{p^{2/p}\Gamma(3/p)}{\Gamma(1/p)}m^{-2/p},
\end{split}
\end{eqnarray*}
where in the "$\approx$" step we have used the expansion $\Gamma((m+2)/p) \approx (m/p)^{2/p}\Gamma(m/p)$, which is valid for large $m/p$. Putting things together, we see that $\lim_{p \rightarrow \infty}\dfrac{p^{2/p}\Gamma(3/p)}{\Gamma(1/p)}m^{-2/p} = 1/3$, i.e $\sigma_{m,\infty}^2 = 1/3$, and that
$$
\sigma_{m,p}^2 = \frac{p^{2/p}\Gamma(3/p)}{\Gamma(1/p)}m^{-2/p} \le \begin{cases}2m^{-2/p},&\mbox{ if }1 \le p < 2,\\m^{-2/p},&\mbox{ if }2 \le p < \infty\end{cases}
$$
\end{proof}

\subsubsection{Spectral bounds for AND coefficients}
\begin{restatable}[AND coefficient versus Frobenius norm]{lm}{spectum}
Given a matrixit holds that
$A \in \mathbb R^{k \times m}$, it holds that
\begin{eqnarray}
\alpha_{m,k,p,q}\Delta_{p,q}(A) \le \|A\|_F,
\end{eqnarray}
where
\begin{eqnarray}
 \alpha_{m,k,p,q} :=  k^{-\theta_{q,2}}\cdot \begin{cases}(1/\sqrt{2})m^{1/p},&\mbox{ if }1 \le p < 2,\\m^{1/p},&\mbox{ if }2 \le p < \infty,\\\sqrt{3},&\mbox{ if }p=\infty.\end{cases}
\label{eq:spectum}
\end{eqnarray}
and the exponents $\theta_{\cdot,\cdot} \in [0, 1]$ are as defined in \eqref{eq:thetapq}.
\label{lm:spectum}
\end{restatable}

\begin{proof}
By Lemma \ref{lm:lpcov}, $u$ has zero mean and covariance matrix $\sigma_{m,p}^2I_m$ where
$$
\sigma_{m,p}^2 = \cdot \begin{cases}2m^{-2/p},&\mbox{ if }1 \le p < 2,\\m^{-1},&\mbox{ if }2 \le p < \infty,\\1/3,&\mbox{ if }p=\infty\end{cases}
$$ 
Thus, one computes
\begin{eqnarray}
\mathbb E_u\|Au\|_2^2 = \trace(A^TA\Sigma_p) = \sigma_{m,p}^2\|A\|_F^2 = \|A\|_F^2\cdot \begin{cases}2m^{-2/p},&\mbox{ if }1 \le p < 2,\\m^{-2/p},&\mbox{ if }2 \le p < \infty,\\1/3,&\mbox{ if }p=\infty.\end{cases}
\label{eq:covtrace}
\end{eqnarray}

On the other hand, by Lemma \ref{lm:lpequiv}, one has
$\|Au\|_q \le k^{\theta_{q,2}}\|Au\|_2$.
Taking expectations on both sides and using \eqref{eq:covtrace}, we then get
\begin{eqnarray*}
\begin{split}
\frac{\Delta_{p,q}(A)}{\|A\|_F} &\le k^{\theta_{q,2}}\begin{cases}\sqrt{2}m^{-1/p},&\mbox{ if }1 \le p < \infty,\\1/\sqrt{3},&\mbox{ if }p=\infty.\end{cases}\\
\end{split}
\end{eqnarray*}
which is nothing but the recriprocal of \eqref{eq:spectum}.
\end{proof}

\begin{restatable}[Induced $p/q$ matrix-norms]{df}{}
Given a matrix $A \in \mathbb R^{k \times m}$, we have the bound, the induced matrix-norm of $A$, denoted $\|A\|_{p,q}$ is defined by
$$
\|A\|_{p,q} = \sup_{\|x\|_p \le 1}\|Ax\|_q.
$$
Note that, since $A$ can be seen as a linear operator from the normed vector-space $\ell_p^m$ to the normed vector-space $\ell_q^k$, $\|A\|_{p,q}$ is precisely an instance of the operator norm defined in Definition \ref{df:pqnorm}.
\end{restatable}

For simplicity, when $p=q$, we will denote $\|A\|_{p,p}$ by $\|A\|_p$ (single subscript).

\begin{restatable}[Upper bound on induced $p/q$ matrix-norms in terms of spectral norm]{lm}{pqonspec}
Given a matrix $A \in \mathbb R^{k \times m}$, we have the bound
\begin{eqnarray}
\|A\|_{p,q} \ge \frac{k^{\theta_{2,q}}}{m^{\theta_{p,2}}}\|A\|_2,
\end{eqnarray}
where the exponents $\theta_{\cdot,\cdot} \in [0, 1]$ are as defined in \eqref{eq:thetapq}.
\label{lm:pqonspec}
\end{restatable}
\begin{proof}
Let $x \in \ell_p^m$ (nonzero). Then, by Lemma \ref{lm:lpequiv}, we have
\begin{eqnarray*}
\begin{split}
\|x\|_p &\le m^{\theta_{p,2}}\|x\|_2,\text{ i.e }\frac{1}{\|x\|_p} \ge \frac{1}{m^{\theta_{p,2}}\|x\|_2},\text{ and }\\
\|Ax\|_q &\ge k^{\theta_{2,q}}\|Ax\|_2.
\end{split}
\end{eqnarray*}
Multiplying both inequalities then gives
$$
\frac{\|Ax\|_q}{\|x\|_p} \ge \frac{k^{\theta_{2,q}}\|Ax\|_2}{m^{\theta_{p,2}}\|x\|_2}.
$$
In then suffices to max-out $x$ on both sides to get the result via Definition \eqref{eq:pqnorm}
\end{proof}

In particular, taking $p=q \in \{1,\infty\}$ begets the following corollary.

\begin{restatable}{cor}{}
Given a matrix $A \in \mathbb R^{k \times m}$, we have the boundss
\begin{eqnarray}
\|A\|_\infty \ge \sqrt{k}\|A\|_2, \;\|A\|_1 \ge \frac{1}{\sqrt{m}}\|A\|_2.
\end{eqnarray}

\end{restatable}
\begin{restatable}[Induced $p/q$ matrix-norms versus AND coefficient]{thm}{}
Given a matrix $A \in \mathbb R^{k \times m}$, we have the bound, we have the following bounds
\begin{eqnarray}
\begin{split}
\frac{\|A\|_{p,q}}{\Delta_{p,q}(A)} &\ge \frac{\|A\|_2}{\|A\|_F}\cdot k^{1/2-1/q}\cdot\begin{cases}
(1/\sqrt{2})m^{1/2},&\mbox{ if }1 \le p < 2,\\
m^{1/p},&\mbox{ if }2 \le p < \infty,\\
\sqrt{3},&\mbox{ if }p=\infty.\end{cases}\\
&\ge \sqrt{\frac{k}{\rank A}}\cdot k^{-1/q}\cdot\begin{cases}
(1/\sqrt{2})m^{1/2},&\mbox{ if }1 \le p < 2,\\
m^{1/p},&\mbox{ if }2 \le p < \infty,\\
\sqrt{3},&\mbox{ if }p=\infty.\end{cases}
\end{split}
\end{eqnarray}
\label{thm:specratio}
\end{restatable}
\begin{proof}
This is a direct consequence of Lemmas \ref{lm:pqonspec} and \ref{lm:spectum}, and the fact that $\|A\|_F \le \sqrt{\rank A}\|A\|_2$.
\end{proof}

\begin{restatable}{cor}{}
Given a matrix $A \in \mathbb R^{k \times m}$, we have the bound, we have the following bounds
\begin{eqnarray}
\begin{split}
\frac{\|A\|_{p,q}}{\Delta_{p,q}(A)} &\ge \frac{\|A\|_2}{\|A\|_F}\cdot k^{1/2-1/q}\cdot\begin{cases}
(1/\sqrt{2})m^{1/2},&\mbox{ if }1 \le p < 2,\\
m^{1/p},&\mbox{ if }2 \le p < \infty,\\
\sqrt{3},&\mbox{ if }p=\infty.\end{cases}\\
&\ge \sqrt{\frac{k}{\rank A}}\cdot k^{-1/q}\cdot\begin{cases}
(1/\sqrt{2})m^{1/2},&\mbox{ if }1 \le p < 2,\\
m^{1/p},&\mbox{ if }2 \le p < \infty,\\
\sqrt{3},&\mbox{ if }p=\infty.\end{cases}
\end{split}
\end{eqnarray}
\label{thm:specratiospecial}
\end{restatable}
\subsection{Fluctuations of nonlinear functions}
We are now ready to present one of our main contributions.
\begin{restatable}[Adversaries are stronger than noise!]{thm}{}Let $p,q \in [1,\infty]$, $x \in \ell_p^m$, and let the function $h: \ell_p^m \rightarrow \ell_q^k$ be differentiable at $x$. Then we have the bounds
\begin{eqnarray}
\begin{split}
\frac{\Delta_{\max} h(x)}{\overline{\Delta} h(x)} &\ge \frac{\|\nabla h(x)\|_2}{\|\nabla h(x)\|_F}\cdot k^{1/2-1/q}\cdot\begin{cases}
(1/\sqrt{2})m^{1/2},&\mbox{ if }1 \le p < 2,\\
m^{1/p},&\mbox{ if }2 \le p < \infty,\\
\sqrt{3},&\mbox{ if }p=\infty\end{cases}\\
&\ge \sqrt{\frac{k}{\rank \nabla h(x)}}\cdot k^{-1/q}\cdot\begin{cases}
(1/\sqrt{2})m^{1/2},&\mbox{ if }1 \le p < 2,\\
m^{1/p},&\mbox{ if }2 \le p < \infty,\\
\sqrt{3},&\mbox{ if }p=\infty\end{cases}\\
&\ge k^{-1/q}\cdot\begin{cases}
(1/\sqrt{2})m^{1/2},&\mbox{ if }1 \le p < 2,\\
m^{1/p},&\mbox{ if }2 \le p < \infty,\\
\sqrt{3},&\mbox{ if }p=\infty\end{cases}
\end{split}
\end{eqnarray}
\end{restatable}

\begin{proof} Thanks to Lemma \ref{lm:diffble}, we have
\begin{eqnarray}
\begin{split}
\overline{\Delta} h(x) &= \Delta_{p,q}(\nabla h(x)),\\
\Delta_{\max} h(x) &= \|\nabla h(x)\|_{\ell_p^m,\ell_q^k} = \|\nabla h(x)\|_{p,q}.
\end{split}
\end{eqnarray}
Using the above equalities in conjunction of Theorem \ref{thm:specratio} applies to the jacobian matrix $A = \nabla h(x)$ then concludes the proof.
\end{proof}

%\input{lame_proof.Tex}

==> broader_impact.tex <==
\paragraph{Broader impact.}
As AI-powered systems reach human or super-human levels of performance on a
broad array of tasks (natural language processing, drug discovery, robots, face
recognition, recommender systems, etc.), importance, confidence, and investment
is being placed, at times blindly, on these systems. The general narrative of
advocates of this AI-solves-everything movement is that, these "intelligent"
systems will better the overall situation of society and boost the economy.
However, there are a number of fundamental issues which are still unsolved or
not even yet formulated properly. These include questions having to do with
fairness, data-privacy, and accountability of AI-powered systems. All of these
aspects have potential negative impact on peoples' lives. There are also safety
issues that come with self-driving cars, unjustified surveillance of populations
for supposed law-enforcement, technologically-enabled oppression of populations,
etc. The ML and AI communities are now well-aware of all these concerns, and
there is a serious ongoing scientific research program on these questions going
on all over the world, and an attempt to limit the negative footprint of AI on
the planet, and produce truly "intelligent" systems (whether this is realizable
is another question altogether...).

The subject of adversarial attacks and defenses is at the forefront of this
planetary research enterprise, is questioning the very foundations of classical
(supervised) machine-learning theory. With the aforementioned concerns at heart,
our work studies the fundamental limitations of classifiers (the core
"intelligent" component in AI-powered systems). We raise a warning flag on the
possibility that it might simply be impossible to let AI go fully automatics,
without the risk for life-changing disaster in certain situations. It forces a
rethink of our current view on machine learning, and how it relates to the real
world.



==> bug.tex <==
\fix{Bug (typographic) in the statement of Corollary \ref{corr:gausscurve} in
  main manuscript: The
  conclusion reads $$ \err^*_\omega(P^1,P^2) =
  \inf_{(P^1,P^2)}t\left(2\Phi\left(\frac{M^{-1}(\alpha/t)}{\varepsilon}\right)-1\right),
$$ but it should be $$
\inf_{(P^1,P^2)}\err^*_\omega(P^1,P^2) \ge
\frac{1}{2}\left(1-t\left(2\Phi\left(\frac{M^{-1}(\alpha/t)}{\varepsilon}\right)-1\right)\right),
$$
where the infimum is taken over all classification problems $(P^1,P^2)$ such
that $\tv(P^1,P^2) \le t$ and Condition \ref{cond:orlize} is satisfied.
This mistake has been corrected in the restated version of the Corollary in this
supplemental  (see the end of section \ref{subsec:markovy}).
}


==> dro.tex <==
\section{Defense via distributionally robust optimization}
Let $\mathcal Z$ be a polish space, $P$ be a distribution on $\mathcal Z$, and $c:\mathcal Z \times \mathcal Z \rightarrow [0, \infty]$ be l.s.c with $c(z,z) = 0$ for all $z \in \mathcal Z$. Let $\varphi: \mathcal Z \rightarrow \mathbb R$ be u.s.c with $\varphi(z) \le K(1+c(z,z_0))^m$ for some $K,m \ge 0$ and $z_0 \in Z$. For $\varepsilon \ge 0$, let $\err_{P,\varepsilon}^{\text{rob}}(\varphi):=\min_{\ot_c(Q,P) \le \varepsilon}\mathbb E_{z \sim Q}[\varphi(z)]$ Under these conditions, it is known that
\begin{eqnarray}
\err_{P,\varepsilon}^{\text{rob}}(\varphi) = \inf_{\alpha \ge 0}\alpha\varepsilon + \mathbb E_{z \sim P}[\varphi^{\alpha c}(z)],
\end{eqnarray}
where $\varphi^{\alpha c}(z) := \sup_{z' \in \mathcal Z}\varphi(z') - \alpha c(z',z)$. Given an iid sample $z_1,\ldots,z_n \sim P$ of size $n \ge 1$, the goal of this section is to construct an efficient data-driven estimator $\err_{\hat{P}_n,\varepsilon}^{\text{rob}}(\varphi)$ for $\err_{P,\varepsilon}^{\text{rob}}(\varphi)$,
where
\begin{eqnarray}
\err_{\hat{P}_n,\varepsilon}^{\text{rob}}(\varphi) = \inf_{\alpha \ge 0}\alpha\varepsilon + \mathbb E_{z \sim \hat{P}_n}[\varphi^{\alpha c}(z)]=\inf_{\alpha \ge 0}\alpha\varepsilon + \frac{1}{n}\sum_{i=1}^n\varphi^{\alpha c}(z_i).
\end{eqnarray}

\subsection{Ruin probabilities}
Here $\varphi = \mathbbm{1}_E$ for some Borell $E \subseteq \mathcal Z$. One computes
$$
\varphi^{\alpha c}(z) := \sup_{z' \in \mathcal Z}\varphi(z') - \alpha c(z',z)=\sup_{z' \in \mathcal Z}\mathbbm{1}_E(z')-\alpha c(z',z) = (1-\alpha c(z,E))_+,
$$
where $c(z, E):= \inf_{z \in E}c(z,E)$. Thus,
\begin{eqnarray}
\err_{\hat{P}_n,\varepsilon}^{\text{rob}}(\varphi)=\inf_{\alpha \ge 0}\alpha\varepsilon + \frac{1}{n}\sum_{i=1}^n\varphi^{\alpha c}(z_i)=\inf_{\alpha \ge 0}\alpha\varepsilon + \frac{1}{n}\sum_{i=1}^n(1-\alpha d_i)_+,
\end{eqnarray}
where $d_i := c(z_i,E)$.

\begin{restatable}{lm}{optbis}
Let $0 \le d_1 \le d_2 \le \ldots \le d_n$ and $\varepsilon \ge 0$. Define $n_0 := \#\{i \in \{1,\ldots,n\} \mid d_i = 0\}$ and $\gamma := \min_{\alpha \ge 0}f(\alpha)$, where $f(\alpha):=\alpha\varepsilon + \frac{1}{n}\sum_{i=1}^n(1-\alpha d_i)_+$. We have the formula
\begin{eqnarray}
0 \le \gamma = \frac{1}{n}\min(a_\varepsilon, b_\varepsilon) \le f(0)=1,
\end{eqnarray}
where $a_\varepsilon := \min_{n_0 \le i < i_\varepsilon}\left(i + \frac{n\varepsilon - \overline{d}_i}{d_i}\right)$, $b_\varepsilon := \min_{i_\varepsilon \le i \le n}\left(i + \frac{n\varepsilon - \overline{d}_i}{d_{i+1}}\right)$, $d_{n+1}=\infty$,
$\overline{d}_i := \sum_{j=1}^i d_j$ and $i_\varepsilon := \max\{i \in [n_0, n] \mid \overline{d}_i \le \varepsilon\}$.

Moreover, if $\varepsilon \ge (1/n)\sum_{i=1}d_i$, then $\gamma = f(0)=1$.
\label{thm:optbis}
\end{restatable}

\subsection{Adversarial attacks}
Let $c:\mathcal X \times \mathcal X \rightarrow \mathbb R$ be l.s.c such that $c(x,x) = 0$ and define $\tilde{c}:(\mathcal X \times \mathcal Y)^2 \rightarrow [0,\infty]$ by
\begin{eqnarray}
\tilde{c}((x',y'),(x,y)) = \begin{cases}
c(x',x'),&\mbox{ if }y' = y,\\ +\infty,&\mbox{ else.}
\end{cases}
\end{eqnarray}
Let $\ell:\mathcal Y \times \mathcal Y \rightarrow  \mathbb R$ be a loss function. Given a classifier $h:\mathcal X \rightarrow \mathcal Y$, define $\ell_h:\mathcal X \times \mathcal Y \rightarrow \mathbb R$ by $\ell_h(x, y) := \ell(h(x),y)$.
Also define the measurable subset $E_h := \{(x,y) \mid h(x) \ne y\} \subseteq \mathcal X \times \mathcal Y$. Note that $E_h$ can be partitioned like so 
$$
E_h = \cup_{y \in \mathcal Y}(E_{h,y} \times \{y\}),
$$
where $E_{h,y} := \{x \in \mathcal X \mid h(x) = y\}$. Finally, define $\overline{E}_h \subseteq \mathcal X \times \mathcal Y$ by
$$
\overline{E}^c_h := \{(x,y) \mid \tilde{c}((x,y), E) = 0\} = \{(x, y) \mid c(x,E^c_{h,y})=0\}=\cup_{y=1}^K\overline{E}^c_{h,y} \times \{y\},
$$
where $\overline{E}^c_{h,y} := \{x \in \mathcal X \mid c(x,E_{h,y})=0\}$.
and note that
$$
\err_{P,c}(h)=P(\overline{E}^c_{h})=\sum_{y=1}^K P(\overline{E}^c_{h,y} \times \{y\})=\sum_{y=1}^K P_{X|y}(\overline{E}^c_{h,y})P_Y(y).
$$

For example, in the case of metric attacks where $\mathcal X = (\mathcal X, d)$ is a metric space and the ground cost is given by $c(x',x) = \mathbbm{1}[\![d(x',x) > \delta]\!]$, one computes
$
\overline{E}^c_{h,y} = \{x \in \mathcal X \mid d(x,E_{h,y}) \le \delta\} = E_{h,y}^{\delta}$, the $\delta$-enlargement of $E_{h,y}$.
Thus in this case, we have
\begin{eqnarray}
P_{X|y}(\overline{E}^c_{h,y})=P_{X|y}(d(X,E_{h,y}) \le \delta) = P_{X|y}(\exists x' \in \ball(X;\delta) \mid h(x') \ne y).
\end{eqnarray}

\begin{theorem}
Let $c:\mathcal X \times \mathcal X \rightarrow [0,\infty)$ be a symmetric l.s.c cost function such that $c(x,x) \equiv 0$. For a loss function $\ell:\mathcal Y \times \mathcal Y \rightarrow [0, 1]$ and a classifier $h:\mathcal X \rightarrow \mathcal Y$, define the robust risk  $\err_{P,\varepsilon}^{\rob}(\ell_h):=\sup_{\ot_{\tilde{c}}(Q,P) \le \varepsilon}\mathbb E_Q[\ell_h(x,y)]$, where $\ell_h(x,y) := \ell(h(x),y)$. Then
\begin{itemize}
    \item For the binary loss $\ell(y',y) := \mathbbm{1}[\![y' \ne y]\!]$, we have
\begin{eqnarray}
\err_{P,\varepsilon}^{\rob}(\ell_h) = \sup_{\ot_{c}(Q,P) \le \varepsilon}Q(E_{h}) = \mathbb E_{P_Y}\left[\inf_{\alpha \ge 0}\alpha\varepsilon + \mathbb E_{P_{X|y}}[(1-\alpha c(X,E_{h,y}))_+]\right],
\label{eq:magic}
\end{eqnarray}
where as before, $E_{h,y} := \{x \in \mathcal X \mid h(x) \ne y\}$ and $E_h := \cup_{y}E_{h,y}\times \{y\}$, and $c(x,E_{h,y}) := \inf_{x' \in E_{h,y}}c(x',x)$. % Moreover, there is equality in \eqref{eq:magic} if $\varepsilon \ge \mathbb E_{P_{X|y}}[c(X,A)]$.
\item If $c$ is a binary cost, then
\begin{eqnarray}
\err_{P,\varepsilon}^{\rob}(\ell_h) = \mathbb E_{P_Y}\left[\inf_{\alpha \ge 0}\alpha\varepsilon + \mathbb E_{P_{X|y}}[\max(\widetilde{\ell}_h(x,y),M_y-\alpha)]\right],
\end{eqnarray}
where $\widetilde{\ell}_h(x,y):=\underset{x' \in \mathcal X \mid c(x',x) = 0}{\sup}\ell_h(x',y) \le M_y := \underset{x' \in \mathcal X}{\sup}\ell_h(x',y) \le 1$.
\end{itemize}
\end{theorem}

\begin{definition}[Covering number of a hypothesis class]
Let $\mathcal H \subseteq \mathbb R^{\mathcal X}$ be a collection of hypotheses and $n$ be a positive integer and $t > 0$. The covering number of $\mathcal H$ is defined by
$$
\mathcal N_\infty(\mathcal H, t, n):= \sup_{(x_1,\ldots,x_n) \in \mathcal X^n}\mathcal N(\mathcal H(x_1,\ldots,x_n),t,\|\cdot\|_\infty),
$$
where $\mathcal H(x_1,\ldots,x_n) := \{(f(x_1),\ldots,f(x_n)) \mid f \in \mathcal H\} \subseteq \mathbb R^n$, and for $A \subset \mathbb R^n$, is the number of $\mathcal N(A,t,(\mathbb R^n,\|\cdot\|_\infty))$ is the minimum number of $\ell_\infty$ balls of radius $t$ needed to cover $A$.
\end{definition}

\begin{lemma}[Covering number of Lipschitz composition]
Let $\mathcal H \subseteq \mathbb R^{\mathcal X}$ be a collection of hypotheses and $\Phi \subseteq \mathbb R^{\mathbb R}$ be a collection of $\rho$-Lipschitz functions. Then
$$
\mathcal N_\infty(\Phi \circ \mathcal H, t,n)=\mathcal N_\infty(\mathcal H,t/\rho,n),
$$
where $\Phi \circ \mathcal H := \{\varphi \circ h \mid \varphi \in \Phi,\; h \in \mathcal H\} \subseteq \mathbb R^{\mathcal X}$.
\end{lemma}

\begin{lemma}[Uniform empirical Bernstein inequality]
Let $\mathcal H \subseteq \mathbb R^{\mathcal X}$ be a collection of hypotheses and let $\mathcal M_{\mathcal H}(n) := 10\mathcal N(\mathcal H, 1/n,2n)$. For every $n \ge 16$ and $\delta \in (0, 1)$, it holds w.p $1-\delta$ uniformlly for all $h \in \mathcal H$ that
\begin{eqnarray}
 |\mathbb E_{P}[h] - \mathbb E_{\hat{P}_n}[h]| \le \sqrt{\frac{18V_n(h)\log(\mathcal M_{\mathcal H}(1/n,2n)/\delta)}{n}} + \frac{15\log(\mathcal M_{\mathcal H}(1/n,2n)/\delta)}{n-1},
\end{eqnarray}
where $\mathcal M_{\mathcal H}(t,m) := 10\mathcal N_\infty(\mathcal H,t,m))$, and $V_n(h)$ is the empirical variance of $h$.
\end{lemma}

\begin{corollary} Let $M>0$ and $\ell:\mathbb R \times \mathbb R \rightarrow [0, M]$ be a loss function and $\mathcal H \subseteq \mathbb R^{\mathcal X}$ be a collection of hypotheses. For $h \in \mathcal H$, define $\ell_h:\mathcal X \times \mathbb R \rightarrow [0, M]$ by $\ell_h(x, y) = \ell(h(x),y)$. Then for every $n \ge 16$, $\varepsilon \ge 0$ and $\delta \in (0, 1)$, w.p $1-\delta$, it holds uniformly for all $h \in \mathcal H$ that
\begin{eqnarray}
\begin{split}
|\err_{P,\varepsilon}^{\rob}(\ell_h) - \err_{\hat{P}_n,\varepsilon}(\ell_h)| &\le 
\sqrt{\frac{18V_n(h)\log(\mathcal M_{\mathcal H}(\frac{\varepsilon}{nM},2n)/\delta)}{n}} + \frac{15\log(\mathcal M_{\mathcal H}(\frac{\varepsilon}{nM},2n)/\delta)}{n-1}\\
&= \frac{M}{\varepsilon}\sqrt{\frac{18\log(\mathcal M_{\mathcal H}(\frac{\varepsilon}{nM},2n)/\delta)}{n}} + \frac{15\log(\mathcal M_{\mathcal H}(\frac{\varepsilon}{nM},2n)/\delta)}{n-1}.
\end{split}
\end{eqnarray}
\end{corollary}
\begin{proof} For $h \in \mathcal H$ and $\alpha \ge 0$, define $\psi_{P,\varepsilon,h}(\alpha) := \alpha\varepsilon + \mathbb E_P[\ell_h^{\alpha c}]$.
Let $\hat{\alpha}(h) = \hat{\alpha}_{n,\varepsilon}(h) := \argmin_{\alpha \ge 0}\psi_{\hat{P}_n,\varepsilon,h}(\alpha)$. Then
\begin{eqnarray*}
\begin{split}
\err_{P,\varepsilon}^{\rob}(\ell_h)-\err_{\hat{P}_n,\varepsilon}^{\rob}(\ell_h) &:= \inf_{\alpha \ge 0}\psi_{P,\varepsilon,h}(\alpha)-\inf_{\alpha \ge 0}\psi_{P,\varepsilon,h}(\alpha) = \inf_{\alpha \ge 0}\psi_{P,\varepsilon,h}(\alpha)-\psi_{\hat{P}_n,\varepsilon,h}(\hat{\alpha}(h))\\
&= \psi_{P,\varepsilon,h}(\hat{\alpha}(h))-\psi_{\hat{P},\varepsilon,h}(\hat{\alpha}(h))
\le \mathbb E_{P}[\ell_h^{\hat{\alpha}(h) c}]-\mathbb E_{\hat{P}_n}[\ell_h^{\hat{\alpha}(h) c}].
\end{split}
\end{eqnarray*}
Consider the collection of hypotheses $\mathcal F_{n,\varepsilon} := \{\ell_h^{\hat{\alpha}_n(h)} \mid h \in \mathcal H\}$
\end{proof}

\begin{restatable}{lm}{opt}
Let $a \in \mathbb R$ and $-\infty < c_1 \le c_2 \le \ldots \le c_n \le b$.
Then
\begin{eqnarray}
\min_{x \le b}\;ax + \sum_{i=1}^n|c_i-x| = \overline{c}_n+\min\left(\min_{0 \le i \le (n-a)/2}d_ic_{i+1} - 2\overline{c}_i,\min_{(n-a)/2 < i \le n}d_ic_{i} - 2\overline{c}_i\right),
\end{eqnarray}
where $c_0:=-\infty$, $c_{n+1}=b$, $\overline{c}_i := \sum_{i=1}^n c_i$ and $d_i := a + 2i - n$, for every $i=1,\ldots,n$.
\label{thm:opt}
\end{restatable}

\begin{restatable}{lm}{realopt}
Let $-\infty < a_1 \le a_2 \le \ldots \le a_n \le  b < \infty$. For $1 \le i \le n$, let $\alpha_i := b - a_i$ and $\overline{\alpha}_j := \sum_{j=1}^i\alpha_j$.
If $\alpha_1 > 0$ (i.e $a_1 < b$), let $n_0 = \max\{i \in \{1,\ldots,n\} \mid \alpha_i > 0\}$. For every $\varepsilon \ge 0$, define $\Delta_{n,\varepsilon}$ by
\begin{eqnarray*}
\begin{split}
n\Delta_{n,\varepsilon} &:=
\begin{cases}\underset{0 \le i \le n_0}{\min}(\overline{\alpha}_i + \min((n\varepsilon-i)\alpha_{i+1},(n\varepsilon-i)\alpha_i)),&\mbox{ if }\alpha_1 > 0,\\
0,&\mbox{ else,}
\end{cases}\\
&= \begin{cases}\min\left(\underset{0 \le i \le \min(n_0,\lfloor n\varepsilon\rfloor)}{\min}\bar{\alpha}_i + (n\varepsilon-i)\alpha_{i+1},\underset{\lfloor n\varepsilon\rfloor + 1 \le i \le n_0}{\min}\bar{\alpha}_i + (n\varepsilon-i)\alpha_i\right),&\mbox{ if }\alpha_1 > 0,\\
0,&\mbox{ else,}
\end{cases}
\end{split}
\end{eqnarray*}
where $\overline{\alpha}_0:=0$ and $\alpha_{n_0+1}=0$. Then $0 \le \Delta_{n,\varepsilon} \le \varepsilon(b-a_1)$ and we have the identity
\begin{eqnarray}
\begin{split}
\inf_{\alpha \ge 0}\alpha\varepsilon + \frac{1}{n}\sum_{i=1}^n\max(a_i,b-\alpha)
= \frac{1}{n}\sum_{i=1}^na_i+\Delta_{n,\varepsilon}=\frac{1}{n}\sum_{i=1}^na_i+\mathcal O(\varepsilon).
\end{split}
\label{eq:nice}
\end{eqnarray}
\end{restatable}

\begin{figure}
\includegraphics[width=.5\linewidth]{opt.png}
\includegraphics[width=.5\linewidth]{optbis.png}
\caption{Graphical illustration of Lemmas \ref{thm:opt} and \ref{thm:optbis}.}
\end{figure}

\subsection{Proofs of lemmas}
\opt*
\begin{proof}
Let $f(x) := ax + \sum_{i=1}^n|c_i-x|$ and $\gamma := \min_{x \le b}f(x)$. Since
$-\infty =: c_0 < c_1 \le c_2 \le \ldots c_n \le c_{n+1} := b$, the domain of optimization can be partitioned as $ (-\infty, b] = \cup_{i=1}^n (c_i,c_{i+1}]$, and so $\gamma = \min_{0 \le i \le n} f_i$, where
$$
f_i := \inf_{c_i < x \le c_{i+1}} ax + \sum_{i=j}^n|c_j-x|.
$$
For $1 \le i \le n$, define $\overline{c}_i := \sum_{j=1}^ic_j$, and set $\overline{c}_0 := 0$. For any $i \in \{0,1,\ldots,n\}$, one computes,
\begin{eqnarray*}
\begin{split}
f_i &:= \inf_{c_i < x \le c_{i+1}} ax + \sum_{j=1}^n|c_j-x| = \inf_{c_i < x \le c_{i+1}} ax + \sum_{j=1}^i(x-c_j) + \sum_{j=i+1}^n(c_j-x)\\
&=\inf_{c_i < x \le c_{i+1}} (a+2i-n)x+\overline{c}_n-2\overline{c}_i = \overline{c}_n-2\overline{c}_i + \min((a+2i-n)c_i,(a+2i-n)c_{i+1}).
\end{split}
\end{eqnarray*}
Note that if $a \ge n$, then $f_0 = \min((a-n)c_0,(a-n)c_{1}) + \overline{c}_n=-\infty$, since $c_0 := -\infty$. This explains the initial requirement that $a \le n$. Further, one notes that $d_i \ge 0 \iff i \le (n-a)/2$.
Putting things together, we get the analytic formula

\begin{eqnarray*}
\begin{split}
\gamma &=\min_{0 \le i \le n}f_i=\overline{c}_n+\min\left(\min_{0 \le i \le (n-a)/2}(a+2i-n)c_{i+1} - 2\overline{c}_i,\min_{(n-a)/2 < i \le n}(a+2i-n)c_{i} - 2\overline{c}_i\right).\\
\end{split}
\end{eqnarray*}
%All in all, the complexity of the computations are $\mathcal O(n)$ (including the complexity of presorting the $c_i$'s!).
\end{proof}

\optbis*
\begin{proof}
By definition of $n_0$, the sequence $d=(d_0,d_1,\ldots,d_n,d_{n+1})$ satisfies.

$$
0=:d_0=\ldots=d_{n_0} < d_{n_0+1} \le \ldots d_{n} < d_{n+1} := \infty.
$$
Thus, $f(\alpha)=\alpha\varepsilon + \frac{n_0}{n}+\sum_{i=n_0+1}^n(1-\alpha d_i)_+$.
Now, define $\alpha_i := \alpha_i \in [0, \infty]$ for $i=n_0,\ldots, n+1$, and note that $0=\alpha_{n+1} < \alpha_n \le \ldots < \alpha_0 = \infty$. Thus, the domain of optimization $[0,\infty)$ can be partitioned as follows
$$
[0, \infty] = [0, \alpha_n) \cup [\alpha_n,\alpha_{n-1}) \cup \ldots \cup [\alpha_{n_0+2},\alpha_{n_0+1}) \cup [\alpha_{n_0+1},\infty) = \cup_{i=n_0}^n[\alpha_{i+1},\alpha_i).
$$
Now, one computes $n\gamma-n_0 := n\min_{\alpha \ge 0}f(\alpha)-n_0=\min_{n_0 \le i \le n}f_i$,
where
\begin{eqnarray*}
\begin{split}
f_i &:= \min_{\alpha_{i+1} \le \alpha < \alpha_i}n\varepsilon\alpha + \sum_{j=n_0+1}^i(1-\alpha d_j)_+=\min_{\alpha_{i+1} \le \alpha < \alpha_i}n\varepsilon\alpha + \sum_{j=n_0+1}^i(1-\alpha d_i)\\
&= i-n_0 + \min_{\alpha_{i+1} \le \alpha < \alpha_i}(n\varepsilon-\overline{d}_i) = (i-n_0) + \begin{cases}(n\varepsilon-\overline{d})\alpha_{i+1},&\mbox{ if }\overline{d}_i \le n\varepsilon,\\ (n\varepsilon-\overline{d})\alpha_i,&\mbox{ else.}\end{cases}
\end{split}
\end{eqnarray*}
\end{proof}

\realopt*
\begin{proof}
The goal is to minimize as a function of $\alpha \in [0,\infty)$, the convex piecewise linear function defined by $f(\alpha) := \varepsilon\alpha + \frac{1}{n}\sum_{i=1}^n\max(a_i,b-\alpha)_+$. The domain of optmization in $\alpha$ can be partitioned as $[0,\infty] = \cup_{i=0}^{n_0}[\alpha_{i+1},\alpha_i)$. It is clear that if $\alpha = 0$ (i.e $a_1=\ldots a_n=b$), then $\min_{\alpha \ge 0}f(\alpha)=\frac{1}{n}\sum_{i=1}^na_i$. Otherwise, we have $\min_{\alpha \ge 0}f(\alpha) = \min(f_0,\ldots,f_{n_0})$,
where $f_i := \min_{\alpha_{i+1} \le \alpha < \alpha_i} f(\alpha)$.
Now, since $\alpha_i:=b - a_i$, we have $\max(a_i,b-\alpha)=a_i + (b-\alpha-a_i)_+ = a_i + (\alpha_i-\alpha)_+$. Thus, for $0 \le i \le n_0$, one computes
\begin{eqnarray*}
\begin{split}
nf_i &:= \min_{\alpha_{i+1} \le \alpha < \alpha_i}n\varepsilon\alpha + \sum_{j=1}^n(a_j + (\alpha_j-\alpha)_+)=\sum_{j=1}^n a_j +\sum_{j=1}^n(\alpha_j-\alpha)_+\\
&=\sum_{j=1}^n a_j +\min_{\alpha_{i+1} \le \alpha < \alpha_i}n\varepsilon\alpha +\sum_{j=1}^i (\alpha_j-\alpha) = \sum_{j=1}^n a_j +\min_{\alpha_{i+1} \le \alpha < \alpha_i}n\varepsilon\alpha +\sum_{j=1}^i (\alpha_i-\alpha)\\
&=\sum_{i=1}^n a_i +\min_{\alpha_{i+1} \le \alpha < \alpha_i}(n\varepsilon-i)\alpha + \overline{\alpha}_i = \sum_{j=1}^n a_j + \overline{\alpha}_i+\begin{cases}(n\varepsilon-i)\alpha_{i+1},&\mbox{ if }i \le \lfloor n\varepsilon\rfloor,\\
(n\varepsilon-i)\alpha_i,&\mbox{ else,}\end{cases}
\end{split}
\end{eqnarray*}
which gives formula \eqref{eq:nice}. Plugging $i=0$ in first term of the min defining $\Delta_{n,\varepsilon}$, we get $\Delta_{n,\varepsilon} \le (n\varepsilon-0)\alpha_{0+1}=n\varepsilon\alpha_1=n\varepsilon(b-a_1)$, which completes the proof.
\end{proof}


==> gausscurve.tex <==
There are numerous consequences for supervised
machine learning. The following corollary is the most natural one.
\begin{restatable}[Universal bound under isotropic Gaussian noise]{cor}{gausscurve} Consider
  the isotropic Gaussian kernel $\omega_x = \mathcal N(x,\varepsilon^2 I)$ on a (possibly
  infinite-dim.) euclidean space $\mathcal X$.
% Let $\|.\|$ be any norm on $\mathbb R^m$.
  Then, $\forall t \in (0, 1]$ and classification problem $(P^1,P^2) \in
  \mathcal G_{M,\alpha}(t)$, we have
\begin{eqnarray}
\err^*_\omega(P^1,P^2) =
\frac{1}{2}\left(1-
  t\left(2\Phi\left(\frac{M^{-1}(\alpha/t)+\Delta}{\varepsilon}\right)-1\right)\right).
% \le t\sqrt{1-e^{-\frac{1}{\pi}(M^{-1}(\alpha/t)/\varepsilon)^2}}
\label{eq:gausscurve}
\end{eqnarray}
where $\Delta := \|\mu_1-\mu_2\|$ and $\Phi$ is the standard Gaussian CDF.%  In
% particular, for      %
% $\mathcal X=(\mathbb R^m,\|\cdot\|_2)$, we have                    %
% \begin{eqnarray}                                                   %
% \inf_{(P^1,P^2) \in \mathcal S_{m,c}(t)}\err^*_\omega(P^1,P^2) =   %
% \frac{1}{2}\left(1-                                                %
%   t\left(2\Phi\left(c/\varepsilon\right)-1\right)\right).          %
% % \le t\sqrt{1-e^{-\frac{1}{\pi}(M^{-1}(\alpha/t)/\varepsilon)^2}} %
% \label{eq:gausscurvecube}                                          %
% \end{eqnarray}                                                     %

% where $C_{\|\cdot\|}(r) := \max_{\|x\| \le r}\|x\|_2$. 
  \label{corr:gausscurve}
\end{restatable}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{restatable}[Universal bound under uniform noise]{cor}{}                                        %
% Given a classification problem $(P^1,P^2)$ on $\mathbb R^m$, consider a random                        %
% corruption corresponding to the uniform Markov kernel given by $\omega_x :=                           %
% \unif(\ball_\infty(x;\varepsilon))$. Then, $\forall t \in (0, 1]$ we have                             %
% \begin{eqnarray}                                                                                      %
% \inf_{(P^1,P^2)}\err^*_\omega(P^1,P^2) \ge                                                            %
% \frac{1}{2}\left(1-  t\left(1-\exp\left(-\frac{mM^{-1}(\alpha/t)}{2\varepsilon}\right) \right)\right) %
% \label{eq:gausscurve}                                                                                 %
% \end{eqnarray}                                                                                        %
% where the inf. is over all classification problems                                                    %
%  $(P^1,P^2)$ for which $\tv(P^1,P^2) \le t$ and Condition \ref{cond:orlize}                           %
% \end{restatable}                                                                                      %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proof}
By ~\cite[Theorem 1]{barsov87}, we know that
\begin{eqnarray}
\begin{split}
\tv(\omega_x,\omega_{x'}) = \tv(\mathcal N(x,\varepsilon^2 I),\mathcal N(x',\varepsilon^2 I))
= 2\Phi\left(\|x-x'\|/(2\varepsilon)\right) - 1.
\end{split}
  \label{eq:tvgauss}
\end{eqnarray}
We may take $\bar{\theta}^{cc}(r) = \bar{\theta}(r) = \theta(r) =
2\Phi(r/(2\varepsilon))-1\;\forall r \ge 0 $ in Thm. \ref{thm:kingkong} to get
$$
\mathfrak D_{\omega,M,\alpha}(t) \le
t\left(2\Phi\left(\frac{M^{-1}(\alpha/t) + \Delta}{\varepsilon}\right)-1\right),
$$
for all $(P^1,P^2) \in \mathcal G_{M,\alpha}(t)$. Plugging the above bound into
\eqref{eq:noisyrisk} then gives \eqref{eq:gausscurve}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Finally, in the case of classification problems on $\mathbb R^m$ with $(P^1,P^2)     %
% \in \mathcal S_{m,\alpha}$, we may take $x_0 = 0$ and $M(r) := r^p$ and $\alpha      %
% = \max_{k=1,2}\mathbb E_{x \sim P^k}\|x\|_2^p \le (c\sqrt{m})^p$, from which         %
% $$                                                                                   %
% M^{-1}(\alpha/t) = (\alpha/t)^{1/p} \le ((c\sqrt{m})^p/t)^{1/p} = c\sqrt{m}/t^{1/p}. %
% $$                                                                                   %
% Taking $p \to \infty$, we have $M^{-1}(\alpha/t) \to c\sqrt{m}\cdot \lim_{p \to      %
%   \infty}(1/t)^{1/p} = c\sqrt{m}$ for all $t \in (0, 1]$.                            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{proof}


==> gaussian_model.tex <==
\paragraph{Multivariate gaussians.} As a concrete application of Corollary \ref{thm:tool}, consider the following
problem inspired by \cite{tsipras18} were the classification target is uniformly
distributed on $\{1,2\}$ and the class-conditional distribution of the features
are multi-variate Gaussians with the same covariance matrix for both classes.
More formerly, the joint distribution of $X$ and $Y$ is given by $Y \sim
\Bern(\{1,2\}), \;X|(Y=k) \sim \mathcal{N}(\mu_k, \Sigma)$, where
$\mu_1,\mu_2 \in \mathbb R^m$ and $\Sigma$ is an $m$-by-$m$ psd matrix with
singular values $\sigma_1 \ge \ldots \ge \sigma_m \ge 0$. We have the following
corollary.
\begin{restatable}{cor}{gaussian}
Consider a classification problem $(P^1,P^2)$ on $\mathbb R^m$ with $P^k =
(1/2)\mathcal N(\mu_k,\Sigma)$. For $\ell_\infty$-norm
attacks with budge $\varepsilon$, we have
\begin{eqnarray}
  \err_{\varepsilon}^*(P^1,P^2) \ge 1-\Phi(\Delta(\varepsilon)/2) \ge
  1-\Phi\left(\|s(\varepsilon)\|_2/2\right),
\end{eqnarray}
  where $\Delta(\varepsilon) := \dfrac{\|\Delta\|_{\Sigma^{-1}}}{\varepsilon} =
  \dfrac{\sqrt{\Delta^T\Sigma^{-1}\Delta}}{\varepsilon}$,
  $\Delta := \mu_1-\mu_2 \in \mathbb R^m$, and $s(\varepsilon)
  \in \mathbb R^m$ is defined by $s_j(\varepsilon) :=
  |\sigma_j|^{-1}(|\Delta_j|-\varepsilon)_+$, for all $ j \in [\![m]\!]$.
  \label{thm:gaussian}
\end{restatable}

\input{sample_complexity.tex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Extension to general exponential families.}                                               %
Now consider an exponential family with natural parameter $\theta \in \Theta \subseteq \mathbb R^m$, %
sufficient statistic $T:\mathcal X \in \mathbb R^m$, and density                                     %
\begin{eqnarray}                                                                                     %
f(x;\theta) = b(x)\exp(\theta^T T(x) - F(\theta)).                                                   %
\end{eqnarray}                                                                                       %
The mean parameter is $\mu := \mathbb E_\theta[t(x)]$. One can show that $\mu =                      %
\nabla F(\theta)$.                                                                                   %
It is well-known that the KL divergence between any two members $P_\theta$ and                       %
$P_{\theta'}$ is % given by                                                                            %
\begin{eqnarray}
  \begin{split}
  \kl(P_\theta\|P_{\theta'}) &= F(\theta) -                    %
F(\theta') - (\theta-\theta')^T\nabla F(\theta')\\
&=: B_F(\theta' \| \theta),
\end{split} %
\end{eqnarray}
where $ B_F$ is the Bregman divergence functional generated by $F$. Thus, the by                     %
Pinker-Kullback-Csiszar inequality, one has $\tv(P^1, P_2 + z) \le \kl (P^1 \|
P^2 + z) \le \sqrt{B_F(\widehat{\theta}_2 + z\|\widehat{\theta}_1)}$. Let
$\Delta := \widehat{\theta}_2 - \widehat{\theta}_1$. Because
$B_F$ is convex and $L$-smooth in the first argument, we have
\begin{eqnarray*}
\begin{split}
&\inf_{\|z\| \le \varepsilon}B_F(\widehat{\theta}_2 + z \| \widehat{\theta}_1) \le B_F(\widehat{\theta}_2\|
\widehat{\theta}_1)\\
&\quad\quad\quad + \inf_{\|z\| \le \varepsilon}z^T(\nabla F(\widehat{\theta}_1) - \nabla
F(\widehat{\theta}_2)) + \frac{L}{2}\|z\|^2\\
&\quad= B_F(\widehat{\theta}_2 \| \widehat{\theta}_1) - \frac{\|\Delta\|^2}{2L} +  \inf_{\|z\| \le
  \varepsilon} \frac{L}{2}\|z - \Delta/L\|^2\\
&\quad= B_F(\widehat{\theta}_2 \| \widehat{\theta}_1) - \frac{\|\Delta\|^2}{2L} + \frac{L}{2}\left(
  \frac{\|\Delta\|}{L}-\varepsilon \right)_+^2\\
&\quad = B_F(\widehat{\theta}_2 \| \widehat{\theta}_1) - \begin{cases}\frac{\|\Delta\|^2}{2L},&\mbox{if
  }\|\Delta\| \le
  L\varepsilon,\\\varepsilon\|\Delta\|-\frac{L}{2}\varepsilon^2,&\mbox{else}
\end{cases}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% &\le B_F(\widehat{\theta}_2 \| \widehat{\theta}_1) - \begin{cases}\frac{\|\Delta\|^2}{2L},&\mbox{if %
%   }\|\Delta\| \le                                                                                   %
%   L\varepsilon,\\\frac{L}{2}\varepsilon^2,&\mbox{else}                                              %
% \end{cases}\\                                                                                       %
% &\le B_F(\widehat{\theta}_2 \| \widehat{\theta}_1) - \frac{L}{2}\min(\varepsilon,\|\Delta\|/L)^2    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{split}
\end{eqnarray*}



==> ipm.tex <==
\subsubsection{Extension to other metrics}
\paragraph{Information divergences.}
M. Reid and R. C. Williamnson (e.g see Theorem 10 of ~\cite{ReidW11}) have
expanded the above principle $(1)$ to the case where the TV metric is replaced
with other information divergences $D_f$ generated from other potentials $f$.
For example $f(t) = |t-1|$ for TV; $f(t) = t\log(t)$ for KL divergence; $f(t) =
(\sqrt{t}-1)^2$ for Hellinger distance; $f(t) = (t-1)^2$ for chi-squared
divergence, etc. Each of these divergences generates a corresponding \emph{calibrated}
margin-based loss function $\phi_f$ such that
$
\err^*(P,\phi_f) = \frac{1}{2}(1-D_f(P^1,P^2)),
$
where $\err^*(P,\phi_f) := \inf_{h}\err(h; P, \phi_f)$ is the Bayes risk for the
loss with margin function $\phi_f$.

\paragraph{Integral probability metrics.}
~\cite{ipm09} establishes a link between certain IPMs (Wasserstein, MMD, etc.)
corresponding to symmetric function classes, i.e $-\mathcal H = \mathcal H$, and
certain loss functions in binary classification. Consider the loss function
$\ell:\mathbb R \times \{\pm 1\} \rightarrow \mathbb R$ defined by $\ell(y,y') =
\phi(yy')$, where $\phi:\mathbb R \rightarrow \mathbb R$ is defined by $\phi(t)
= (1-t)/2$. Note that $2 \phi(t) = \phi_{\text{Hinge}}(t) := (1-t)_+$ for $|t|
\le 1$, and so $\phi$ is \emph{Bayes consistent / classification-calibrated} on
classifiers which are bounded.

\begin{restatable}[IPMs as classification risk]{lm}{bayesipm}
Let $\mathcal H$ be a symmetric class of measurable functions (i.e $h \in
\mathcal H \implies -h \in \mathcal H$). Then w.r.t the margin-based loss
$\ell(y',y) = \phi(yy')$ where $\phi(t) := (1-t)/2$, we have the identity:
%\begin{eqnarray}
$\err(\mathcal H;P,\phi) = \dfrac{1}{2}(1-\gamma_{\mathcal H}(P^1,P^2)).
$
% \end{eqnarray}
\label{thm:bayesipm}
\end{restatable}

% \paragraph{Examples.}
As an example, recall that the Wasserstein distance is an IPM corresponding to
taking $\mathcal H = \text{Lip}_1(\mathcal X)$, the space of $1$-Lipschitz
real-valued functions on $\mathcal X$, we get
$$
\err^*(\text{Lip}_1(\mathcal X, \mathbb R);P,\phi) = \dfrac{1}{2}(1-W_1(P^1,P^2)).
$$
Likewise, taking $\mathcal H = \text{BLip}_1(\mathcal X,\mathbb R)$ the space of
all bounded-Lipschitz functions $h:\mathcal X \rightarrow \mathbb R$ with
$\|h\|_{\text{BLip}} := \|h\| + \|h\|_L \le 1$, we have
$$
\err^*(\text{BLip}_1(\mathcal X, \mathbb R);P,\phi) = \dfrac{1}{2}(1-W_1^{1,1}(P^1,P^2)).
$$
Finally, if $\mathcal H = \mathbb B_{\text{RKHS}}$ is the unit ball of an RKHS, then
$$\err^*(\mathbb B_{\text{RKHS}}; P,\phi) = \dfrac{1}{2}(1-\text{MMD}(P^1,P^2)).
$$

==> lame_proof.tex <==
It then remains to further bound the RHS of (2).

{\bfseries \emph{(A)} Euclidean norm.} By rotational symmetry of the euclidean sphere, $\eta_h(x)^T U$ has the same distribution as $U_1$, the first coordinate of the $U$. But it is a classical result that if $m$ is large, for a point drawn uniformly at random on the euclidean $m$-sphere, each of its coordinates is distributed according to $\mathcal N(0,1/m)$. Thus, for any $t > 0$, we have
$\mathbb P(|\eta_h(x)^T U| > t\|n_h(x)\|_2) = \mathbb P(|U_1| > t) \approx \mathbb P(|\mathcal N(0, 1)| \ge t\sqrt{m})$.
Thus, recalling that the expectation of nonnegative random variable $R$ equals $\int_0^\infty \mathbb P(R > t)dt$, we get
\begin{eqnarray}
\begin{split}
\mathbb E|\eta_h(x)^T U| &= \int_0^\infty \mathbb P(|\eta_h(x)^TU| > t)dt \approx  \int_0^\infty \mathbb P(|\mathcal N(0, 1)| \ge t\sqrt{m})dt\\
&= m^{-1/2}\int_0^\infty \mathbb P(|\mathcal N(0, 1)| > t)dt
= m^{-1/2}\mathbb E|\mathcal N(0, 1)| \le m^{-1/2}.
\end{split}
\label{eq:spectral_bound}
\end{eqnarray}

Combining (1), (2) and (3) then gives $\dfrac{\Delta_{\max} h(x)}{\overline{\Delta} h(x)} \ge \sqrt{m}$ as claimed.

{\bfseries \emph{(B)}: Max-norm.} Here, another standard concentration bound for dot product of a deterministic L2-unit vector (here $\eta_h(x)$ and a uniform random vector in the cube $[-1, 1]^m$ tells us that (e.g se the manuscript [1])
$$
\mathbb P(|\eta_h(x)^TU| > t) \le 2e^{-12t^2}.
$$
Therefore, one computes
\begin{eqnarray}
\mathbb E|\eta_h(x)^TU| = \int_0^\infty \mathbb P(|\eta_h(x)^TU| > t)dt \le 2\int_0^\infty e^{-12t^2}dt = 2\int_0^\infty e^{-(\sqrt{24})^2t^2/2}dt=\frac{\sqrt{2\pi}}{\sqrt{24}} = \sqrt{\frac{\pi}{12}}.
\label{eq:cube_bound}
\end{eqnarray}
Combining (1), (2), and (4) then gives $\dfrac{\Delta_{\max} h(x)}{\overline{\Delta} h(x)} \ge \sqrt{m}  \ge \sqrt{\dfrac{\pi}{12}}\dfrac{\|\nabla h(x)\|_1}{\|\nabla h(x)\|_2} > 1.95\dfrac{\|\nabla h(x)\|_1}{\|\nabla h(x)\|_2}$, as claimed.

\subsection{Lipschitz-gradient case}
Suppose $h$ is  differentiable function with $L$-Lipschitz gradient, meaning that
$$
|\nabla h(x') - \nabla h(x)| \le L\|x'-x\|,\;\forall x,x' \in \mathcal X.
$$
This implies the well-known \emph{Lipschitz-gradient inequality}

$$
-\frac{L}{2}\|x'-x\|^2 + \nabla h(x)^T(x'-x) \le h(x') - h(x) \le \nabla h(x)^T(x'-x) + \frac{L}{2}\|x'-x\|^2,\;\forall x,x' \in \mathcal X.
$$


==> noise_proofs.tex <==

\subsection{Proofs for results in section \ref{sec:noise}}
 \label{subsec:markovy}

% \bayesoptomega*
\begin{proof} We prove a more general result for any loss function $\ell:\mathbb
  R\times [\![K]\!] \rightarrow \mathbb R$. Let, $\ell_h(x,y) := \ell(h(x),y)$.
  Recall the definition of the sub-probability measures $P^y$ on $\mathcal X$
  for $y \in [\![K]\!]$. Now, by direct computation, we have
\begin{eqnarray*}
\begin{split}
  \err_\omega(h;P;\ell) &:=
  % \mathbb E_{X,Y}[\mathbb E_{\tilde{x} \sim \omega_X}[\ell_h(\tilde{x},Y)]]
\sum_y \mathbb E_{x \sim P^y}[\mathbb E_{\tilde{x} \sim
  \omega_x}[\ell_h(\tilde{x},y)]] =\sum_y \mathbb E_{x \sim (P^y *
  \omega)}[\ell_h(\tilde{x},y)]  =: \err(\ell_h;P^1 * \omega, P^2 * \omega),
\end{split}
\end{eqnarray*}
which proves the first identity. The result is then a simple consequence of the
classical fact that $\err(Q^1, Q^2)=\frac{1}{2}(1-\tv(Q^1,Q^2))$, applied to the
classification problem $(Q^1,Q^2)=
(P^1 * \omega, P^2 * \omega)$.
\end{proof}

% \bayesipm*
% \begin{proof}
% For this loss, the risk of a classifier $h \in \mathcal H$ writes
% \begin{eqnarray*}
% \begin{split}
% 2\err(h;P;\phi) &= 2\mathbb E_{P_-}[\phi(h(X))] + \mathbb E_{P_+}[\phi(-h(X))] =
% \mathbb E_{P-}[1+h(X)]  + \mathbb E_{P_+}[1 - h(X)]\\ &= \mathbb
% E_{P_-}[1]+\mathbb E_{P_+}[1] + \mathbb E_{P_-}[h(X)] - \mathbb E_{P_+}[h(X)] =
% 1 + \mathbb E_{P_-}[h(X)] - \mathbb E_{P_+}[h(X)],
% \end{split}
% \end{eqnarray*}
% where we have used the elementary fact that $\mathbb E_{P_-}[1]+\mathbb
% E_{P_+}[1]=1$. Thus
% \begin{eqnarray*}
% \begin{split}
% 2\err^*(\mathcal H; P,\phi) - 1 &= \inf_{h \in \mathcal H}\;(2\err(h; P,\phi) -
% 1) = \inf_{h \in \mathcal H}\mathbb E_{P_-}[h(X)] - \mathbb E_{P_+}[h(X)]\\
% &=-\sup_{h\in \mathcal H}\mathbb E_{P_+}[h(X)] - \mathbb E_{P_-}[h(X)]
% \overset{(*)}{=}-\sup_{h\in \mathcal H}|\mathbb E_{P_+}[h(X)] - \mathbb
% E_{P_-}[h(X)]|\\
% &=: -\gamma_{\mathcal H}(P_+,P_-),
% \end{split}
% \end{eqnarray*}
% where (*) is because $-\mathcal H = \mathcal H$. We conclude that
% $\err^*(\mathcal H; P,\phi) = \dfrac{1}{2}(1-\gamma_{\mathcal H}(P_+,P_-))$.
% \end{proof}

% \kingkong*
\begin{proof}
  We upper-bound $\tv(P^1 * \omega, P^2 * \omega)$, the result will follow
  directly from \eqref{eq:bridge}.
  
  Our technique is an adaptation of the proof of ~\cite{polyanskiy16}.
% \paragraph{The upper bound.}
Let $t \in (0, 1]$ and $(P^1,P^2) \in \mathcal G_{M,\alpha}(t)$ with
$\tv(P^1,P^2) \le t$.
We begin by noting that for every $x,x' \in \mathcal X$, one has
$$
\tv(\omega_x,\omega_{x'}) \le \theta(d(x,x')) \le \theta(d(x,\mu_1) + d(x',\mu_2) + d(\mu_1,\mu_2)),
$$
where the 2nd inequality is the triangle inequality for the pseudo-metric $d$.
Thus, for every coupling $(X_1,X_2)$ of $P^1$ and $P^2$, we have
\begin{eqnarray*}
\begin{split}
\tv(P^1 * \omega, P^2 * \omega) &\le \mathbb P(X_1 \ne X_2)(\mathbb E[\theta(d(X_1,\mu_1) + d(X_2,\mu_2) +
d(\mu_1,\mu_2)) \mid X_1 \ne X_2]\\
&\le \mathbb P(X_1 \ne X_2)(\theta(\mathbb E[d(X_1,\mu_1)] + \mathbb E[d(X_2,\mu_2) \mid X_1 \ne X_2] +
d(\mu_1,\mu_2))\\
&= \mathbb P(X_1 \ne X_2)(\theta(\mathbb E[d(X_1,\mu_1) \mid X_1 \ne X_2] + \mathbb E[d(X_2,\mu_2) \mid
X_1 \ne X_2] + d(\mu_1,\mu_2)),
\end{split}
\end{eqnarray*}
where the 2nd inequality is Jensen's inequality. Now, one computes
\begin{eqnarray*}
\begin{split}
&M\left(\frac{\mathbb E[d(X_1,\mu_1) \mid X_1 \ne X_2]}{2} + \frac{\mathbb E[d(X_2,\mu_2) \mid
    X_1 \ne X_2]}{2}\right)\\
&\quad\quad\le \mathbb E\left[M\left(\frac{d(X_1,\mu_1)}{2} +
    \frac{d(X_2,\mu_2)}{2}\right)\bigg | X_1 \ne X_2\right]\\
&\quad\quad= \frac{1}{\mathbb P(X_1 \ne X_2)}\mathbb E\left[M\left(\frac{d(X_1,\mu_1)}{2} +
    \frac{d(X_2,\mu_2)}{2}\right)\right]\\
&\quad\quad\le \frac{1}{\mathbb P(X_1 \ne X_2)}\left(\frac{\mathbb E\left[M(d(X_1,\mu_1)\right]}{2} +
  \frac{\mathbb E\left[M(d(X_2,\mu_2)\right]}{2}\right)\\
&\quad\quad\le \frac{1}{\mathbb P(X_1 \ne X_2)}\left(\frac{\alpha}{2} + \frac{\alpha}{2}\right) =
\frac{\alpha}{\mathbb P(X_1 \ne X_2)},
\end{split}
\end{eqnarray*}
from which $\mathbb E[d(X_1,\mu_1) \mid X_1 \ne X_2] + \mathbb E[d(X_2,\mu_2) \mid X_1 \ne X_2]
\le 2M^{-1}(\alpha/\mathbb P(X_1 \ne X_2))$. Putting things together, we get
\begin{eqnarray*}
\tv(P^1 * \omega, P^2 * \omega) \le \mathbb P(X_1 \ne
  X_2)\left(\theta\left(2M^{-1}\left(\frac{\alpha}{\mathbb P(X_1 \ne
  X_2)}\right)+d(\mu_1,\mu_2)\right)\right).
\end{eqnarray*}
Since the function $s \mapsto s\theta(2M^{-1}(\alpha/s) +
\theta(d(\mu_1,\mu_2)))$ is non-decreasing, optimizing ove the coupling
$(X_1,X_2)$ yields
\begin{eqnarray*}
\begin{split}
\tv(P^1 * \omega, P^2 * \omega) &\le
\tv(P^1,P^2)\left(\theta\left(2M^{-1}\left(\frac{\alpha}{\tv(P^1,P^2)}\right) +
    d(\mu_1,\mu_2)\right)\right) \\
&\le t\left(\theta\left(2M^{-1}\left(\frac{\alpha}{t}\right)+d(\mu_1,\mu_2)\right)\right).
\end{split}
\end{eqnarray*}
where the last inequality is because $\tv(P^1,P^2) \le t$ by hypothesis.%  Since %
% $(P^1,P^2) \in \mathcal G_{M,\alpha}(t)$ was chosen arbitrarily,               %
% \eqref{eq:oneside} holds as claimed.                                           %

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% For the lower bound \eqref{eq:otherside}, indeed, for arbitrary $x_0,x_1,x_2 \in %
% \mathcal X$ such $x_0$ is a midpoint of $x_1$ and $x_2$ and $d(x_1,x_0) \le      %
% M^{-1}(\alpha/t)$, consider the pair of distributions $(P^1, P^2)$ defined by    %
% $                                                                                %
% P^k = (1-t)\delta_{x_0} + t\delta_{x_k}.                                         %
% $                                                                                %
% It is clear that $(P^1,P^2) \in \mathcal G_{M,\alpha}(t)$, because of the        %
% condition $d(x_1,x_0) = d(x_2,x_0)) \le M^{-1}(\alpha/t)$ and the triangle       %
% inequality for $d$. Moreover, it is easy to compute $\tv(P^1,P^2) = t$ and       %
% $\tv(P^1 * \omega, P^2 * \omega) = \tv((1-t)\omega_{x_0} + t\omega_{x_1},        %
% (1-t)\omega_{x_0} + t\omega_{x_2}) =                                             %
% t\tv(\omega_{x_1},\omega_{x_2})=t\theta(d(x_1,x_2))$. Optimizing over            %
% $(x_0,x_1,x_2)$, we get \eqref{eq:otherside}.                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The result then follows directly from \eqref{eq:bridge}.
\end{proof}

% \stablerank*
\begin{proof}
Let $s := m\sigma^2_0$. If $\Sigma_0$ is not positive definite, then it $\Sigma_0$ can
be seen as a limit of positive definite matrices. Thus we may restrict $\Sigma$
to the cone of positive definite matrices. By the method of Lagrange multipliers,
  $$
  \min_{\trace\Sigma \le s}\alpha(\Sigma) = \min_{\trace\Sigma \le
    s}\trace(\Sigma^{-1}\Sigma_0) = \max_{w \ge 0}\min_{\Sigma}\trace(\Sigma^{-1}\Sigma_0) +
  w(\trace\Sigma - s)).
  $$
  Differentiating w.r.t $\Sigma$ and setting to zero gives, $-\Sigma^{-2}\Sigma_0 +
  w I_m = 0$, i.e $\Sigma = \Sigma_0^{1/2}/\sqrt{w}$. Furthermore, the constraint
  $\trace\Sigma = s$ yields $w=\trace \Sigma_0^{1/2}/s$, and so $\Sigma = (s/\trace
  \Sigma_0^{1/2})\Sigma_0^{1/2}$. With this choice of $\Sigma$, we have
$s\trace(\Sigma^{-1}\Sigma_0) = (\trace \Sigma_0^{1/2})^2 =
(\trace \Sigma_0^{1/2})^2
= (\sum_{j=1}^r \sqrt{\lambda_j^2})^2 \le r\sqrt{\|\Sigma_0\|_{op}}$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Recall that in classical machine learning (i.e without any noise                       %
% corruption), the Bayes-optimal error is exact $\frac{1}{2}(1-\tv(P^1,P^2))$. In        %
% the noisy case (random corruption), the next result, namely Corollary                  %
% \ref{corr:gausscurve}, gives a quantitative lower bound on noisy Bayes-optimal         %
% error for classification problems of all difficulties, as measured by level curves the %
% total-variation distance between the class-conditional distributions                   %
% $\tv(P^1,P^2)$. The result is illustrated in Fig. \ref{fig:dob}.                       %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \input{bug.tex}



==> note.tex <==
        Corollary \ref{corr:gausscurve} gives a quantitative lower bound on
        Bayes-optimal error for classification problems of all difficulties, as
        measured by level curves the total-variation distance between the
        class-conditional distributions $\tv(P^1,P^2)$. Recall that in classical
      machine learning (i.e without any noise corruption), the Bayes-optimal
      error is exact $\frac{1}{2}(1-\tv(P^1,P^2))$

==> ollivier_ricci.tex <==
\section{The Ollivier-Ricci curvature for metric spaces}
\subsection{Preliminaries}
In classical geometry, Ricci curvature is usually defined as a measure of how close "small balls" are, compared to the distance between their centers. Intuitive, it measures the amount of distortion undergone by the length a small arc joining to points on a manifold, via parallel transport\todo{I should verify that I'm not saying bs here!}. \emph{\textbf{Q:} But how would one sensibly define a notion of curvature for something as "rough" as the Hamming cube $\{0, 1\}^p$, for example ?}

For a general abstract metric space $(\mathcal X,d)$, the key idea in Ollivier's theory of Ricci curvature ~\cite{OllivierRicci} is to replace the construct of "small balls" with the more general construct of prescribing a measure $\omega_x \in \mathcal P(\mathcal X)$ at each point $x$ of $\mathcal X$. Formally,
% \subsubsection{Terminology}



The concepts of \emph{reversible} and \emph{invariant} measures will be crucial in the sequel.

\begin{restatable}[Reversible and invariant measures]{df}{}
Let $(\mathcal X,d,\omega)$ be an RW-metric space. A measure $\mu \in \mathcal M(\mathcal X)$ is said to be
\begin{itemize}
\item \textbf{reversible} if it satisfies the detailed balanced equation
\begin{eqnarray}
\diff \omega_x(x')\diff\mu(x) = \diff \omega_{x'}(x)\diff\mu(x'),\;\forall x,x' \in \mathcal X.
\end{eqnarray}
\item \textbf{invariant} if $\mu$ is an eigenmeasure of $\omega$, i.e
\begin{eqnarray}
\mu * \omega = \mu.
\end{eqnarray}
\end{itemize}
\end{restatable}

The following is a classical lemma which is true even for general Markov kernels (not just random walks as defined here).
\begin{restatable}[]{lm}{revinv}
In an RW-metric space, every reversible measure is invariant.
\label{thm:revinv}
\end{restatable}

\paragraph{Example: $\varepsilon$-step random walk ~\cite{OllivierRicci}.} Let $\varepsilon > 0$ and let $\mu$ be a probability measure on $\mathcal X$ such that $\supp(\mu) = \mathcal X$ and each $\ball_{\mathcal X}(x;\varepsilon) := \{x' \in \mathcal X \mid d(x',x) \le \varepsilon\}$ has $\mu$-volume. Define the random walk $\omega^{\varepsilon,\lambda}$ on $(\mathcal X,d,\mu)$ by
    $$
    \diff \omega^{\varepsilon,\lambda}_x(x') = \begin{cases}\dfrac{\diff\lambda(x')}{\lambda(\ball_{\mathcal X}(x;\varepsilon))},&\mbox{ if }d(x',x) \le \varepsilon,\\ 0, &\mbox{ else.}\end{cases}
    $$
    That is, for each $x \in \mathcal X$, $\omega_x^{\varepsilon,\lambda}$ is the $\lambda$-uniform distribution on $\ball_{\mathcal X}(x;\varepsilon)$. Then $\lambda$ is reversible (and therefore invariant) for $\omega^{\varepsilon,\lambda}$.
    Note that if $\mathcal X$ is a smooth riemannian manifold, then $\diff \omega^{\varepsilon,\lambda}_x = (1 + \mathcal O(\varepsilon^2))\diff vol(x)$, and so the random walk $\omega^{\varepsilon,\lambda}$ is an $\varepsilon$-scale "zoom" on the rienmannian structure of $\mathcal X$.

\subsection{Constructing random walk / reversible probability measure pairs}
\label{sec:pregibbs}
Let $\mu$ be a finite nonnegative measure on a metric space $(\mathcal X,d)$, % that is to say, $(\mathcal X,d,\mu)$ is a metric measure space.
Let $R:\mathcal X \times \mathcal X \rightarrow [0, \infty)$ be a mapping such that for every $x \in \mathcal X$, $R(x,\cdot)$ is measurable, $\mu$-integrable, and zero $\mu$-almost nowhere. Note that these conditions ensure that the expected value $Z_x := \mathbb E_\lambda [R(x,X')]$ is strictly positive and finite for all $x \in \mathcal X$. For each $x \in \mathcal X$, define the mapping $\omega^{R,\lambda}_x:\borel(\mathcal X) \rightarrow \mathcal P(X)$ by
\begin{eqnarray}
    \omega^{R,\lambda}_x(A) = \frac{1}{Z_x}\int_{x' \in A} R(x,x')\diff \lambda(x').
    \label{eq:pregibbs}
\end{eqnarray}
The following theorem is immediate.
\begin{restatable}[]{thm}{jwalk} If for some (and therefore for all) $x_0 \in \mathcal X$ and for every $x \in \mathcal X$ the function $R(x,\cdot)d(x_0,\cdot)$ is $\mu$-integrable, then $(\mathcal X, d, \omega^{R,\lambda})$ is an RW-metric space.
Moreover, if $J$ is symmetric (i.e $R(x,x') = R(x',x)$ for all $x,x' \in \mathcal X$) and $Z_x := \mathbb E_\lambda[R(x,X')]$ is a constant independent of $x$, then
$\mu$ is reversible (and therefore invariant!).
\label{thm:jwalk}
\end{restatable}

We now explore a few examples of reversible measures constructed this way.

\paragraph{Examples.} Below, we give some examples of random walks of the fom $\omega^{R,\lambda}$.
\begin{itemize}
\item \textbf{Static walk.}
Let $(\mathcal X,d,\lambda)$ be a metric measure space and consider the the mapping $R(x,x') = R(x',x)=\delta_x(x')$. One computes $Z_x = \lambda(x)$ for all $x$. This induces the Dirac random (in fact static!) walk $\omega_x(x') = \delta_x(x')$. $\mu$ is clearly reversible for this random walk.

\item \textbf{Deterministic walk.}
Let $(\mathcal X,d,\lambda)$ be a metric measure space, $T:\mathcal X \rightarrow \mathcal X$ be a measurable function, and consider the the mapping $R(x,x') = \delta_{T(x')}(x)$. We have $Z_x = \lambda(T^{-1}(\{x\}))$ for all $x$ and so $\lambda$ is reversible (and therefore invariant) for this random walk iff $T$ is the identity map. Such RW-metric spaces will be important for studying adversarial examples.

\item \textbf{Gaussian random walk.}
For a nontrivial reversible example, consider the Lebesgue measure $\Leb$ on the euclidean space $\mathbb R^p$ and for $t > 0$, take $R_t(x,x') := e^{-t\|x'-x\|^2}$. Then $\omega^{R_t,\Leb}$ is a random walk on $\mathbb R^p$ and $\Leb$ is irreversible (and therefore invariant) for this random walk. 

\item \textbf{Gibbs random walk.}
For a general example, suppose $e^{-td(x_0,.)}$ is $\mu$-integrable for some (and therefore for all!) $x_0$ in $\mathcal X$ and for some $t \ge 0$ (and therefore for all $t' \ge t$). Define $R_t$ by $R_t(x,x') = e^{-td(x,x')}$ for all $x, x' \in \mathcal X$. Then $\omega^{R_t,\lambda}$ is a random walk on $(\mathcal X, d, \lambda)$. Moreover $\lambda$ is reversible (and therefore invariant) for this random walk iff $Z_x:=\mathbb E_\lambda[R_t(x,X')]$ is a constant independent of x.
\end{itemize}

\subsection{Ollivier-Ricci curvature}
The second axiom in the above definition means that each $\omega_x$ belongs to the order-1 Wasserstein space $\mathcal P_1(\mathcal X)$. Thus, one can make sense of $W_1(\omega_x,\omega_{x'}) := \inf_{\gamma \in \Pi(\omega_x,\omega_{x'})}\mathbb E_\gamma[d(X,X')]$, the order-1 Wasserstein distance between $\omega_x$ and $\omega_{x'}$. Ollivier's Ricci curvature is defined in terms of this quantity. Viz,
\begin{restatable}[Ollivier-Ricci curvature]{df}{}
Let $(\mathcal X, d,\omega)$ be an RW-metric space. Given $x,x' \in \mathcal X$, the Ollivier-Ricci curvature $\kappa_\omega(x,x')$ of $\mathcal X$ along the abstract arc $[xx']$ is defined by
\begin{eqnarray}
\kappa_\omega(x,x') := \begin{cases}-\infty, &\mbox{ if }x' = x,\\
1-\dfrac{W_1(\omega_x,\omega_{x'})}{d(x,x')},&\mbox{ else.}\end{cases}
\end{eqnarray}
Given $\kappa \in \mathbb (-\infty, 1]$, we say $(\mathcal X, d, \omega)$ has curvature bound $\kappa$ if $\kappa_w(x,x') \ge \kappa$ for all $x,x' \in \mathcal X$.
\end{restatable}

The following result from  ~\cite{OllivierRicci}, which is proved in the appendix for completeness, will be our main take-away from the Ollivier-Ricci theory.
\begin{restatable}[$W_1$-contraction from curvature bounds]{lm}{contraction}
Let $\kappa \in (-\infty, 1]$. An RW-metric space $(\mathcal X, d, \omega)$ has curvature bound $\kappa$ if and only if $W_1(\mu*\omega,\nu * \omega) \le (1 -\kappa)W_1(\mu,\nu)$ for all $\mu,\nu \in \mathcal P(\mathcal X)$. Moreover, in this case $\mathcal P_1(\mathcal X)$ is preserved by $\omega$, i.e $\mu \in \mathcal P_1(\mathcal X) \implies \mu * \omega \in \mathcal P_1(\mathcal X)$.
\label{thm:contraction}
\end{restatable}
Of course, strictly speaking, have a contraction only when $\kappa > 0$. This result generalizes the well-known Dobrushin-contraction inequality, which corresponds to the particular case when $d$ is the discrete metric: $d(x,x')=\delta_x(x')$.

Lemma \ref{thm:contraction} above can be recovered as a special case of the the following general result, which is more general than the applications we make of it in our manuscript. It is one of our main technical contributions. Viz,

\begin{restatable}[General contraction]{thm}{gc}
Let $ (\mathcal X, d, \omega)$ be an RW metric space. and let $\|\cdot-\cdot\|_D$ be a metric on the measures on $\mathcal X$, and for every pair of measures $\mu$ and $\nu$ on $\mathcal X$, we have
\begin{itemize}
    \item[(A)] General contraction:
\begin{eqnarray}
\|\mu * \omega-\nu * \omega\|_D \le (1-\kappa_{\omega,D})W_d(\mu,\nu),
\end{eqnarray}
where $\kappa_{\omega,D} := 1-\underset{x,x' \in \mathcal X,\;x\ne x'}{\inf}\;\frac{\|\omega_x-\omega_{x'}\|_D}{d(x,x')}$.
\item[(B)] TV-contraction: In particular, taking $d(x,x') := \mathbbm{1}[\![x \ne x']\!]$, the discrete metric, we have
\begin{eqnarray}
\tv(\mu * \omega,\nu * \omega) \le \left(\sup_{x,x'\in\mathcal X,\;x\ne x'}\tv(\omega_x,\omega_{x'})\right)\tv(\mu,\nu).
\end{eqnarray}
\end{itemize}
\label{thm:general_contraction}
\end{restatable}
Lemma \ref{thm:contraction} then corresponds to the special case of part \emph{(A)} where we takke $\|\cdot-\cdot\|_D$ is the 1-Wasserstein distance.
Part \emph{(B)} is nothing but the well-known \emph{Dobrushin data-processing inequality}.

The following is a direct consequence of the above Theorem, to the problem of adversarial examples. Viz,
\begin{restatable}[Adversarial attacks contract information]{thm}{}
Let $P$ be a probability distribution on a bounded subset $\mathcal X$ of $\mathbb R^m$ equipped with an $\ell_p$-norm with $p \in \{2,\infty\}$, and let $\varepsilon > 0$. Then
\begin{eqnarray}
\inf_a \tv(P^+ * a,P^- * a) \le C_{m,p,\varepsilon}\tv(P^+,P^-),
\end{eqnarray}
where
\begin{itemize}
    \item the infimum is taken over all stochastic bounded metric adversaries $a$, with budget $\varepsilon$, i.e markov kernels $a:\mathcal X \rightarrow \mathcal P(\mathcal X)$ such that $\underset{x \in \mathcal X}{\inf}\;\mathbb P_{\tilde{x} \sim a_x}\left(\|\tilde{x}-x\|_p \le \varepsilon\right)=1$, and
    \item The contraction constant $C_{m,p,\varepsilon}$ is given by
$$C_{m,p,\varepsilon}=\begin{cases}I_{(\frac{\diam(\mathcal X)}{2\varepsilon} \land 1)^2}\left(\frac{1}{2},\frac{m+1}{2}\right),&\mbox{ if }p=2,\\
1-\left(1-\frac{\diam(\mathcal X)}{2\varepsilon}\right)_+^m,&\mbox{ if }p=\infty.\end{cases}
$$
\end{itemize}
\end{restatable}
\begin{proof}[Sketch of proof]
Consider the "random jump" kernel $a = \omega^{\Leb,\varepsilon}$, i.e each $a_x$ is the uniform distribution on the $\ell_p$-ball of radius $\varepsilon$ around $x$. It is clear that $\supp(a_x)=\ball_p(x;\varepsilon)$ and so $\inf_{x}\mathbb P_{\tilde{x} \sim a_x}(\|\tilde{x}-x\|_p \le \varepsilon)$. Now, if $x,x' \in \mathcal X$ with $\|x-x'\|_p \ge 2\varepsilon$, then the balls of center $x$ and $x'$ donnot intersect, and so $\tv(a_x,a_{x'})=1$. Otherwise, $1-\tv(a_x,a_{x'})$ equals the the volume of the lens of intersection between these balls, divided by the volume of an either of the balls (the balls have same volume, by invariance of Lebesgue measure). But it is a standard computation that this ratio of volumes is exactly equal to $
I_{1-(\frac{d(x,x')}{2\varepsilon})^2}\left(\frac{m+1}{2},\frac{1}{2}\right)$.
\end{proof}

\subsection{Information contraction for almost-bounded stochastic attackers}
The above theorem is highly restrictive because it only works for bounded feature spaces, and the constants $C_{m,p,\varepsilon}$ are close to 1 except for very low-dimensional regimes. In turns out that we can remove both restrictions by allowing for attacks which can violate the norm-constraint with small probability. This is the case if, for example, the attacker is allower to add untruncated Gaussian corruptions of a given variance (as opposed to adding noise with bounded norm).

For $p \in \alpha,\beta > 0$, and an $L$-Lipschit function $T:\mathcal X \rightarrow \mathcal X$, consider attacks given by Markov kernels of the form \begin{eqnarray}
a_x(\tilde{x}) \propto e^{-\frac{\|\tilde{x}-T(x)\|_\beta^\beta}{\alpha}}.
\end{eqnarray}
For example, the case $(T,\alpha,\beta)=(Id,2\sigma^2,2)$ corresponds to Gaussian corruption. One can prove that
\begin{itemize}
    \item $\mathbb P_{\tilde{x} \sim a_x}(\|\tilde{x}-x\|_\infty \le \varepsilon) \ge 1- \frac{m}{\sigma\varepsilon}e^{-\frac{\varepsilon^2}{2\sigma^2}}$
\end{itemize}
\subsubsection{Some curvature bounds}
\begin{restatable}[TV-contraction for $\omega^{R,\lambda}$ random walks]{thm}{curvebound}
Let $(\mathcal X, \lambda)$ be a measure space and let $R:\mathcal X \times \mathcal X \rightarrow [0,\infty)$ be a function which meets the conditions in the definition of the random walk $\omega^{R,\lambda}$ in \ref{eq:pregibbs} of section \ref{sec:pregibbs}, for the discrete distance $d(x,x') := \mathbbm{1}[\![x' \ne x]\!]$. If there exists $u \in [1,\infty)$ such that
\begin{eqnarray}
\frac{R(x,x')}{R(\tilde{x},x')} \le u,\;\forall x,x',\tilde{x} \in \mathcal X,
\label{eq:ratio}
\end{eqnarray}
then we have the TV-contraction
\begin{eqnarray}
\tv(\mu * \omega^{R,\lambda},\nu * \omega^{R,\lambda}) \le \frac{u^2-1}{u^2+1}\tv(\mu,\nu),\;\forall \mu,\nu \in \mathcal P(\mathcal X).
\end{eqnarray}
\end{restatable}
People from the "differential privacy" community will immediately recognise the
condition \eqref{eq:ratio} is equivalent to saying that the randomized mechanism
$\omega^{R,\lambda}$ is $2\log(u)$-\emph{differentially private}

\subsection{Proofs of technical lemmas and theorems}
\revinv*
\begin{proof}
Let $(\mathcal X, d, \omega)$ be an RW-metric space and $\mu \in \mathcal M(\mathcal X)$ be a reversible measure thereupon. Let $A \subseteq \mathcal X$ be Borel. One computes
\begin{eqnarray*}
\begin{split}
(\mu * \omega)(A) &:= \int_{x \in \mathcal X}\int_{x' \in A}\diff\omega_x(x')\diff\mu(x) \overset{(a)}{=} \int_{x \in \mathcal X}\int_{x' \in A}\diff\omega_{x'}(x)\diff\mu(x')\\
&\overset{(b)}{=} \int_{x' \in A}\left(\int_{x \in \mathcal X}\diff\omega_{x'}(x)\right)\diff\mu(x') \overset{(c)}{=} \int_{x' \in A}1\diff\mu(x') = \mu(A),
\end{split}
\end{eqnarray*}
where \emph{(a)} is an application of Fubini's theorem; \emph{(b)} is by the definition of reversibility of $\mu$; \emph{(c)} is because $m_x$ is a probability measure on $\mathcal X$. Thus, we have shown that $\mu * \omega =\mu$, i.e $\mu$ is invariant.
\end{proof}

\jwalk*
\begin{proof}
Since $\mu \in \mathcal P(\mathcal X)$, it is clear from \eqref{eq:pregibbs} that $m_x^{J,\mu}$ depends measurably on $x$, and for each $x \in \mathcal X$, $\omega^{J,\mu}_x$ is a nonnegative measure with $\omega^{J,\mu}_x(\mathcal X) = 1$, i.e $\omega_x^{J,\mu} \in \mathcal P(\mathcal X)$. If in addition $J(x,\cdot)d(x_0,\cdot)$ is $\mu$-integrable, then $\omega^{J,\mu}$ is indeed a random walk on $(\mathcal X, d)$.

As for the second part of the theorem, this follows by direct computation and the definition of reversibility. Indeed, for every $x,x' \in \mathcal X$ one computes
\begin{eqnarray*}
\begin{split}
\diff\omega_x^{J,\mu}(x')\diff\mu(x) &= \frac{1}{Z_x}J(x,x')\diff\mu(x')\diff\mu(x)
= \frac{1}{Z_x}J(x',x)\diff\mu(x)\diff\mu(x') \\
&= \frac{Z_{x'}}{Z_x}\diff\omega_{x'}^{J,\mu}(x)\diff\mu(x')=\diff\omega_{x'}^{J,\mu}(x)\diff\mu(x'),
\end{split}
\end{eqnarray*}
since $Z_x = Z_{x'}$.
\end{proof}

\curvebound*

\begin{proof}
Let $x,\tilde{x},x' \in \mathcal X$. First note that \eqref{eq:ratio} implies $Z_x := \mathbb E_{\mu}[R(x,X')] \le u\mathbb E_{\mu}[R(\tilde{x},X')]=uZ_{\tilde{x}}$, and so $Z_x/Z_{\tilde{x}} \le u$. Combining this with \eqref{eq:ratio}, we get
$
\dfrac{\diff\omega_x(x')}{\diff\omega_{\tilde{x}}(x')}=\dfrac{Z_{\tilde{x}}}{Z_x}\dfrac{R(x,x')}{R(\tilde{x},x')} \le u^2,
$ from where it follows be Lemma \ref{thm:basic} that
\begin{eqnarray}
\frac{|\diff\omega_x(x')-\diff\omega_{\tilde{x}}(x')|}{\diff\omega_x(x')+\diff\omega_{\tilde{x}}(x')} \le \frac{u^2-1}{u^2+1}.
\end{eqnarray}
Thus, one computes

\begin{eqnarray*}
\begin{split}
\tv(\omega_x,\omega_{\tilde{x}}) &= \frac{1}{2}\int_{x' \in \mathcal X}|\diff\omega_x(x')-\diff\omega_{\tilde{x}}(x')| = \frac{1}{2}\int_{x' \in \mathcal X}\frac{|\diff\omega_x(x')-\diff\omega_{\tilde{x}}(x')|}{\diff\omega_x(x')+\diff\omega_{\tilde{x}}(x')}(\diff\omega_x(x')+\diff\omega_{\tilde{x}}(x'))\\
&\le\frac{1}{2}\frac{u^2-1}{u^2+1}\int_{x' \in \mathcal X}(\diff\omega_x(x')+\diff\omega_{\tilde{x}}(x')) = \frac{u^2-1}{u^2+1}.
\end{split}
\end{eqnarray*}
Applying Corollary \ref{thm:dobrushin} then gives the result.
\end{proof}

\begin{restatable}[]{lm}{basic}
\label{thm:basic}
If $a,b > 0$ and $c \ge 1$, then $\dfrac{a}{b} \le c$ iff $\dfrac{|a-b|}{a+b} \le \dfrac{c-1}{c+1}$.
\end{restatable}
\begin{proof}
WLOG, suppose $a \ge b$.
Then

$$
\frac{|a-b|}{a+b} \le \frac{c-1}{c+1} \iff \frac{a-b}{a+b} \iff \frac{c-1}{c+1} \iff (c+1)(a-b) \le (c-1)(a+b) \iff a \le bc.
$$
\end{proof}

==> sdpi.tex <==
\section{Universal bounds for random corruption}
\label{sec:noise}
We now analyse what happens when the attacker is replaced with a random noise
corruption mechanism. % as in Fig. \ref{fig:awgn}.
For example, think of measurement errors in collected data, or natural dirt on
road traffic signs (this can be problematic for the artificial vision system on
board a self-driving car). Robustness of classifiers to random
perturbations of inputs has been studied as a proxy of their robustness to
adversarial attacks (e.g ~\cite{gilmernoise}). We do not claim that deep
learning is vulnerable to random noise. Of course, certain deep-learning
architectures are known to be robust / invariant w.r.t to certain kinds of noise
of transformations~\cite{scatt}.
One can cite scattering networks as a prime
example. Rather, our goal in this section is to establish quantitative bounds on
adversarial error of any classifier (including deep learning models), as
a function of the size of the noise.

We take an information-theoretic point of view and think of the scenario as that
of transmitting information via a noisy communication channel as in Fig.
\ref{fig:awgn}. For the analysis, we develop strong \emph{Data Processing
  Inequalities (DPIs)} that bound the transmission rate contractively. Already
the basic / weak DPI, we know that a random noise corruption mechanism would
only reduce the total-variation distance between class-conditional
probabilities (making the classification problem harder), and so increase
Bayes-optimal error for the problem. We will provide quantitative
problem-specific lower-bounds which reflect the increase Bayes-optimal error
due to the noise corruption.
% Our strong DPIs make this degradation in performance quantitative.
% on this
                                %  decreased total-variation. % Our results
                                %  extend beyond Gaussian case.

% In turns out that in general, one has to lift the classical notion of
% adversarial attacks to incorporate allow for uncertainty for the attackers
% output. That is invoked twice on the input, the attacker operates different
% modifications on the input, modifications which are chosen at random according
% to some probability distribution. This can be formalized using the notion of a
% random-walk.
\vspace{.2cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{mdframed}                                                                                %
%   \emph{{\bfseries Teaser: the existence of transferable universal adversarial perturbations.}} %
%   As a remarkable application, the results of this section will be                              %
%     used in section \ref{sec:uap} to prove the existence (under the moment                      %
%     constraints \ref{cond:orlize}) of so-called universal                                       %
%     at adversarial perturbations (UAPs): a fixed perturbation vector in $\mathbb R^m$           %
%     with norm $\mathcal O(\sqrt{m})$, which simulatenously fools all classifiers                %
%     on a positive fraction of the data.                                                         %
% \end{mdframed}                                                                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Markov kernels as a model for random corruption}
\label{subsec:markov}
% \begin{restatable}[Markov kernels]{df}{}
%   Let $\mathcal X$ be a measurable space.
\emph{Markov kernels} play a central role in the differential
geometry of very general metric spaces e.g graphs. For example, see
~\cite{OllivierRicci} for a synthetic theory of ricci curvature, built using
Markov kernels. Markov kernels are a generalization of a \emph{Markov chains}.
Intuitively, given a point $x \in \mathcal X$, the distribution $\omega_x$, prescribes
how to "jump" from a point $x$. If $Q$ is a measure on $\mathcal X$,
then the probability of starting at a point $x \sim Q$, and then
landing in a Borel $A \subseteq \mathcal X$ is given by the \emph{convolution}
% % \vspace{-.1cm}
\begin{eqnarray}
(Q * \omega)(A) :=
\int_{x \in \mathcal X}\omega_x(A)\diff Q(x)
= \int_{x \in \mathcal X}\int_{\tilde{x} \in A}\diff \omega_x(\tilde{x})\diff
  Q(x).
  \label{eq:convolution}
\end{eqnarray}
% The measure $\mu * \omega$ is called the convolution of $\mu$ with the Markov kernel $\omega$.
\input{awgn.tex}
More formally, a Markov kernel on $\mathcal X$ is a map
$\omega:\mathcal X \rightarrow \mathcal P(\mathcal X)$, $x \mapsto \omega_x$
such that $\omega_x$ depends measurably on $x$, i.e for every Borel $A \subseteq
\mathcal X$ and every Borel $I \subseteq \mathbb R$, the set $\{x \in \mathcal X
\mid \omega_x(A) \in I\}$ is a Borel subset of $\mathcal X$. $\omega$ can be
seen as a linear operator acting on distributions according to
\ref{eq:convolution}.
% \footnote{This axiom will be crucial for applying
%  \emph{Fubini's Theorem}}.
    %\item For every $x \in \mathcal X$, $\omega_x \in \mathcal P_1(\mathcal X)$.
% \end{itemize}
% Such a triplet $(\mathcal X, d, \omega)$ will be referred to as a Markov kernel metric space, or "RW-metric space" for short.
% \end{restatable}
In particular, note that $\delta_x * \omega = \omega_x\;\forall x \in \mathcal
X$.
% Such a corruption model was also considered in ~\cite{gilmernoise}.
The trivial Markov kernel given by setting $\omega_x = \delta_x\;\forall x \in \mathcal
X$ of course corresponds to classical machine learning with no noise corruption
of the input data. A less trivial example is the \emph{isotropic} Gaussian
Markov kernel (in a possibly infinite-dimensional Hilbert space), for which
$\omega_x \equiv \mathcal N(x,\varepsilon^2 I) = x + \mathcal N(0,\varepsilon^2
I)$.
Refer to Fig. \ref{fig:awgn}.

\paragraph{Links with classical adversarial attacks.} It should be noted that our Markov
kernel model of corruption is general enough to encompase even adversarial
attacks considered in sections \ref{sec:background}, \ref{sec:variational}, and
\ref{sec:distbased}. Indeed, an attacker $a:\mathcal X \rightarrow \mathcal X$
can be encoded as a Markov kernel $\omega^a$ given by $\omega^a_x :=
\delta_{a(x)}$. Thus, adversarial attacks are special cases of noise corruption
in our framework of Markov kernels.
However, this link is only anecdotal because, for the bounds we obtain in this
section, we require the Markov kernel $\omega$ to have (w.r.t Lebesgue), which
is not the case for singular kernels like $\omega^a$. This is not an issue per se,
since in section \ref{sec:distbased} we already obtained explicit bounds in case
of distance-based adversarial attacks.
\begin{restatable}[Misclassification error under random corruption]{df}{}
  Consider a classification problem $(P^1,P^2)$. % Refer to section
  % \ref{sec:bayesian} for terminology.
  Given
  a Markov kernel % (aka stochastic adversarial attack)
  $\omega$ on $\mathcal X$,
  the noisy test error of a classifier $h:\mathcal X \rightarrow
 \{1,2\}$ under corruption by $\omega$
 %, denoted $\err_\omega(h;P)$,
 is defined by
% \begin{eqnarray}
$\err_\omega(h;P^1,P^2) = \sum_{k=1}^2\mathbb E_{x \sim P^k,\;\tilde{x} \sim
  \omega_x} [\mathbbm{1}[\![h(\tilde{x})\ne k]\!]]$.
%\end{eqnarray}
The noisy Bayes-optimal error under corruption by $\omega$ is defined by
%\begin{eqnarray}
$\err^*_\omega(P^1,P^2) := \inf_{h}\err_\omega(h; P^1,P^2)$.
%\end{eqnarray}
\end{restatable}
\begin{restatable}[]{lm}{bayesoptomega}
For any classifier $h:\mathcal X \rightarrow \{1,2\}$, we have the identity
% \begin{eqnarray}
% \label{eq:bayeshomega}
$\err_\omega(h;P^1,P^2) = \err(h;P^1_\omega, P^2_\omega)$,
% \end{eqnarray}
where $P^k_\omega := P^k * \omega$.
Furthermore, it holds that
% \begin{eqnarray}
$\err_\omega^*(P^1,P^2) = \frac{1}{2}(1-\tv(P^1_\omega, P^2_\omega)).$
%\label{eq:bayesoptomega}
%\end{eqnarray}.
\label{lm:bayesoptomega}
\end{restatable}
% % \vspace{-.5cm}

Thus, the game of obtaining universal bounds in the presence of random      %
corruption of inputs is reduced to the study of transmission rates in noisy %
channels.                                                                   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Elementary universal bounds for random corruption}
Henceforth let $d$ be a pseudo-metric on the feature space $\mathcal X$. Refer
to definition \ref{df:metricspace}. We will need the following notion of
regularity of Markov kernels.

\begin{restatable}[Regularity of Markov kernels]{cond}{lips}
Given a measurable function
$\theta:\mathbb R_+ \rightarrow (0, 1]$, a Markov kernel $\omega$ on $\mathcal
X$ is said to be $\theta$-regular iff
% \begin{eqnarray}
$\tv(\omega_x,\omega_{x'}) \le \theta(d(x,x')),\;\forall x,x' \in \mathcal X.$
%\label{eq:condition}
%\end{eqnarray}
\label{cond:lips}
\end{restatable}
% % \vspace{-.52cm}
As we shall see, the above condition is a key ingredient for obtaining strong
DPIs. As an example, consider the Gaussian smoothing Markov kernel given by
$\omega_x = \mathcal N(x,\varepsilon^2 I_m)$. From ~\cite[Theorem 1]{barsov87},
we know that
% \begin{eqnarray}
%\begin{split}
$\tv(\omega_x,\omega_{x'}) = \tv(\mathcal N(x,\varepsilon^2 I),\mathcal N(x',\varepsilon^2 I))
= 2\Phi\left(\|x-x'\|/(2\varepsilon)\right) - 1.$
%\end{split}
% \label{eq:tvgauss}
%\end{eqnarray}
So we can take $\theta(r): = 2\Phi(r/(2\varepsilon)) - 1$ for $r \ge 0$, a concave
nondecreasing function, and Condition \ref{cond:lips} will be satisfied.
%(with equality!).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{restatable}[Strong DPIs from moment conditions]{thm}{mydpi}                            %
% Let $\omega$ be a Markov kernel on $\mathcal X$ and let $d:\mathcal X^2                       %
% \rightarrow [0,\infty)$ be a measurable function. Finally, let $\theta: \mathbb               %
% R_+ \rightarrow (0, 1]$ be a convex non-decreasing function such that Condition               %
% \ref{cond:lips} is satisfied. Then, for any strictly-increasing convex function               %
% $M:\mathbb [0,\infty) \rightarrow [0,\infty]$, and for all $P^1,P^2 \in \mathcal P_{M         %
%   \circ d}(\mathcal X)$, it holds that                                                        %
% % \begin{eqnarray}                                                                            %
% $\tv(P^1 * \omega,P^2 * \omega) \le \theta(W_{M,d}(P^1,P^2)),$                                %
% % \end{eqnarray}                                                                              %
% where                                                                                         %
% % \begin{eqnarray}                                                                            %
% $W_{M,d}(P^1,P^2) := M^{-1}\left(\inf \mathbb E [M(d(X_1,X_2))]\right)$                       %
% %\label{eq:W}                                                                                 %
% % \end{eqnarray}                                                                              %
% and the infimum is taken over all couplings $(X_1,X_2)$ of the distributions $P^1$ and $P^2$. %
% \label{thm:mydpi}                                                                             %
% \end{restatable}                                                                              %
% \begin{proof}                                                                                 %
%   Let $(X_1,X_2)$ be a coupling of $P^1$ and $P^2$. Then                                      %
%   $$                                                                                          %
%   \tv(P^1 * \omega, P^2 * \omega) \le \mathbb P(X_1 \ne X_2)\mathbb                           %
%   E[\theta(d(X_1,X_2)) \mid X_1 \ne X_2] \le \theta(\mathbb E[d(X_1,X_2) \mid X_1 \ne X_2]).  %
%   $$                                                                                          %
%   Also,                                                                                       %
%   \begin{eqnarray*}                                                                           %
%     \begin{split}                                                                             %
%   M(\mathbb E[d(X_1,X_2)) \mid X_1 \ne X_2]) &\le \mathbb E[M(d(X_1,X_2)) \mid                %
%   X_1 \ne X_2]\\                                                                              %
%   \le \frac{1}{\mathbb P(X_1 \ne X_2)}\mathbb E[M(d(X_1,X_2))] ...                            %
%   \todo{Bullshit result; reformulate!}                                                        %
% \end{split}                                                                                   %
%   \end{eqnarray*}                                                                             %
% \end{proof}                                                                                   %
%                                                                                               %
% \begin{restatable}[]{cor}{}                                                                   %
% Let $\mathcal X$, $\omega$, $\theta$ be as in Thm. \ref{thm:mydpi}, with the                  %
% added condition that $d$ is upper-semicontinuous. For every $P^1,P^2 \in                      %
% \mathcal P_{d^p}(\mathcal X)$, we have                                                        %
% % \begin{eqnarray}                                                                            %
% $\tv(P^1 * \omega, P^2 * \omega) \le \theta(W_{d,p}(P^1,P^2))$,                               %
% %\end{eqnarray}                                                                               %
% where $W_{d,p}(P^1,P^2)$ is the $p$-Wasserstein distance between $P^1$ and                    %
% $P^2$, for the ground cost $d$.                                                               %
% \end{restatable}                                                                              %
% \begin{proof}                                                                                 %
% Take $M(r) := r^p$ for all $r \ge 0$ and invoke Theorem \ref{thm:mydpi}, and                  %
% note that $W_{M,d}=W_{p,d}$, the $p$-Wasserstein distance between $P^1$ and                   %
% $P^2$, for the ground cost $d$.% This is actually a distance since $d$ is                     %
% % lower-semicontinuous.                                                                       %
% \end{proof}                                                                                   %
%                                                                                               %
% The above corollary takes us to the right direction: we link the degree of                    %
% separation distributions $P^1 * \omega$ and $P^2 * \omega$ in the smoothed                    %
% problem, measured in total-variation, to the degree of separation between the                 %
% distributions $P^1$ and $P^2$ in the original problem, measured in Wasserstein                %
% distance. However, we are still missing a link to the ultimate complexity                     %
% parameter of the original problem, namely the total-variation between $P^1$ and               %
% $P^2$. Such a link is unlikely to be obtainable from the above corollary as                   %
% there is in general no nonvacuous inequalities between TV and Wasserstein                     %
% metrics (except for extreme cases where the underlying metric space is discrete               %
% and bounded).                                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Blind adversarial attacks as noise channels}
% \begin{restatable}[Blind stochastic adversarial attacks]{df}{}
% A blind adversarial attack is a Markov kernel of the form $\omega_x = P_{Z+x}$ where $Z$ is a $\mathbb R^m$-valued random variable with distribution $P_Z$. We also define the function $\theta_Z:\mathbb R^m \rightarrow [0, 1]$ by
% \begin{eqnarray}
% \theta_Z(x) = \tv(P_Z,P_{Z+x}),
% \end{eqnarray}
% and let $\bar{\theta}_Z$ be the concave envelope of the function $s \mapsto \sup_{\|z\| \le s}\theta_Z(x)$
%{c} \label{def:blinddef}
% \end{restatable}

% \begin{restatable}[Elementary properties of the functions $\theta_Z$ and $\bar{\theta}_Z$]{lm}{}
% Consider a blind attack $\omega$ with noise distribution $P_Z$, and let $\theta_Z$ and $\bar{\theta}_Z$ be as in Definition \ref{def:blinddef}. Then
% \begin{itemize}
%     \item[(A)] {\bfseries Continuity:} $\theta_Z$ is continuous on $\mathbb R^m$, $\theta_Z(0)=0$, $\theta_Z(-x)=\theta_Z(x)$ for all $x \in \mathbb R^m$.
%     \item[(B)] {\bfseries TV control:} $\tv(\omega_x,\omega_{x'}) = \theta(x-x') \le \bar{\theta}_Z(\|x-x'\|)$.
% \end{itemize}
% \label{lm:blinddef}
% \end{restatable}

% \begin{restatable}[Bounds blind stochastic adversarial attacks]{cor}{}
% Consider a blind stochastic attack $\omega_x = P_{Z + x}$. Let $\bar{\theta}_Z$ be the concave envelope of the function
% $s \mapsto \bar{\theta}_Z(s) := \sup_{\|z\| \le s}\theta_Z(z)$, for $s \in \mathbb R^+$. Define the cost $c(x,x') := \|x-x'\|$.
% Then for any strictly-increasing convex function $u:[0,\infty) \rightarrow [0,\infty)$, and for all $P^1,P^2 \in \mathcal P_{u \circ c}(\mathcal X)$, it holds that
% \begin{eqnarray}
% \tv(P^1 * \omega, P^2 * \omega) \le \bar{\theta}_Z(W_{c,u}(P^1,P^2))),
% \end{eqnarray}
% where $W_{c,u}(P^1,P^2))$ is a defined in \eqref{eq:W}.
% \label{thm:blind}
% \end{restatable}

% \begin{proof}
% Note that by Lemma \ref{lm:blinddef}\emph{(B)}, one has
% $\tv(\omega_x,\omega_{x'}) = \theta(x-x') \le \bar{\theta}_Z(\|x-x'\|)=\bar{\theta}_Z(c(x,x'))$. Now apply Thm. \ref{thm:mydpi} with $\theta = \bar{\theta}_Z$.
% \end{proof}

% \subsection{Tight bounds for corruption by smoothing}
% The main kind of Markov kernel we will consider here are of the form $\omega_x = P_{Z+x}$ for some $\mathbb R^m$-values random variable $Z$ whose distribution function $P_Z$ has density of the form $p_Z(z) = \theta(\|z\|)$. Here $\|\cdot\|$ is any norm on $\mathbb R^m$ (e.g $\ell_1$, $\ell_2$, $\ell_\infty$, etc.). Such walks are called \emph{centrally symmetric} as the probability of jumping from $x$ to $x'$ is $\theta(\|x-x'\|)$ which only depends on the distance between $x$ and $x'$. When the norm is $\|.\|_2$ and $\theta(r):=e^{-\frac{1}{2\varepsilon^2}r^2}$, we recover the Gaussian Markov kernel discussed above. When the norm is $\|.\|_1$ and $\theta(r):=e^{-\frac{1}{\varepsilon}r}$, the corresponding Markov kernel is known as a \emph{Laplacian Markov kernel}, as it implements Laplacian smoothing.

% %Note that for a centrally symmetric Markov kernel, we have $\theta_Z(x)=\mathbb P(\|Z\| \le x/2)$.
% \begin{lemma}[Bounds for centrally-symmetric Markov kernels] Suppose $\mathcal X=\mathbb R^m$ equipped with a norm $\|\cdot\|$ and a centrally symmetric Markov kernel given by $\omega_x \equiv P_{Z+x}$ where $Z$ is an $\mathbb R^m$-valued random variable with distribution $P_Z$. For all $P^1,P^2 \in \mathcal P_p(\mathbb R^m)$, we have
% \begin{itemize}
%     \item[(A)] {\bfseries Centrally symmetric noise distribution:} 
% If the noise distribution $P_Z$ has density of the form $p_Z (z)=\theta(\|z\|)$ for some non-increasing function $\theta:[0,\infty) \rightarrow [0,\infty)$.
% \begin{eqnarray}
% \tv(P^1 * \omega,P^2 * \omega) \le \mathbb P\left(\|Z\| \le \frac{1}{2}W_p(P^1,P^2)\right).
% \end{eqnarray}
% \item[(B)] {\bfseries Compactly supported input distributions:} If  $P^1$ and $P^2$ are supported on $\ball(0,R)$, then we have the contraction
% \begin{eqnarray}
% \tv(P^1 * \omega,P^2 * \omega) \le \eta_Z(R)\tv(P^1,P^2),
% \end{eqnarray}
% where $\eta_Z(R) := \sup_{\|z\| \le R}\theta_z(z)$.
% \end{itemize}
% \end{lemma}

% \begin{proof}\emph{(A)} One can prove that under the symmetry hypotheses, it holds that \begin{eqnarray}
% \bar{\theta}_Z(s) = \cdf_{2\|Z\|}(s):=\mathbb P(\|Z\| \le s/2),\;\forall s \in [0,\infty).
% \end{eqnarray}
% One then computes $\tv(\omega_x,\omega_{x'}) \le \bar{\theta}_Z(\|x-x'\|) \le \mathbb P(\|Z\| \le \|x-x'\|/2)$, which is a concave non-increasing function of $\|x-x'\|$. The result then follows from Corollary \ref{thm:blind} with $u(s): = s^p$, and note that $W_{c,u}(P^1,P^2)=W_p(P^1,P^2)$, the $p$-Wasserstein distance induced by the norm $\|.\|$.
% \end{proof}

% \begin{restatable}[Bounds from uniform random smoothing]{cor}{} Let $\mathcal X = \mathbb R^m$ equipped with a norm $\|\cdot\|$ and let $W_1$ (resp. $\mathcal P^1(\mathcal X)$) denote 1-Wasserstein distance (resp. space) induced by the cost the norm. For all $P^1,P^2 \in \mathcal P^1(\mathcal X)$, we have the following bounds
% \begin{itemize}
%     \item[(A)] {\bfseries Uniform random smoothing:}
% For the uniform random smoothing attack $\omega$ given by $\omega_x = P_{\varepsilon Z+x}$ with $\varepsilon > 0$ and $P_Z=\mathcal U(\ball(0;1))$, we have the bound
% \begin{eqnarray}
% \tv(P^1 * \omega,P^2 * \omega) \le \theta\left(\frac{W_p(P^1,P^2)}{2\varepsilon} \land 1 \right),
% \end{eqnarray}
% where $\theta(t) := \begin{cases}I_{t^2}\left(\frac{1}{2},\frac{m+1}{2}\right),&\mbox{ if }\|.\|\text{ is the }\ell_2\text{-norm},\\ 1-(1-t)^m,&\mbox{ if }\|.\|\text{ is the }\ell_\infty\text{-norm}.\end{cases}$
% \item[(B)] {\bfseries Gaussian random smoothing:} %\todo{Not sure what norm I should be using here!}
% For the Gaussian attack $\omega_x = P_{\varepsilon Z+x}$ with $\varepsilon>0$ and $P_Z:=\mathcal N(0,I_m)$,
% we have the bound
% \begin{eqnarray}
% \begin{split}
% \tv(P^1 * \omega,P^2 * \omega) & \le 2M\left(\frac{W_p(P^1,P^2)}{2\varepsilon}\right) - 1.
% \end{split}
% \end{eqnarray}
% \end{itemize}
% \end{restatable}

\subsection{Main results: universal bounds via total-variational Dobrushin curves}
Information theorists know that in general, the TV-based data-processing
inequalities are not contractions. That is, an inequality of the form
$\tv(P^1 * \omega, P^2 * \omega) \le c \tv(P^1, P^2)$ is generally only true
for $c=1$. If we could have $c < 1$, then in view of Theorem
\ref{thm:great}, such a contraction would immediate lead to universal
results of the form: "if ordinary learning on a binary classification problem
$P=(P^1,P^2)$  is hard, then adversarially-robust learning is much harder!".
Lack of contraction is really not a problem. Afterall, all we need are
inequalities of the form $\tv(P^1 * \omega, P^2 * \omega) \le \mathfrak
D(\tv(P^1, P^2))$, for suitable functions $\mathfrak D: [0, 1] \rightarrow [0,
1]$
% (to be prescribed later)
such that $\mathfrak D(t) < t$. Note that if
$\tv(P^1,P^2) \le t$, then the Bayes-optimal error is at least $(1-t)/2$ in the
noiseless regime, and as a consequence of Lemma \ref{lm:bayesoptomega},
% \begin{eqnarray}
$\err^*_\omega(P^1,P^2) \ge
\frac{1}{2}(1-\mathfrak D(t))$,
% \end{eqnarray}
in the noisy regime we consider here. Thus, upper bounds on $\mathfrak
D(t)$ immediately induce lower bounds on bayes-optimal error in the corrupt.
regime. A quantity which can play the rule of such a nonlinear operator
$\mathfrak D$ is given by the theory of nonlinear strong DPIs developed
by Polyanskiy and co-workers~\cite{polyanskiy16} will be the inspiration for the
work in the rest of this section.

\begin{restatable}{df}{}
Given $t \in (0, 1]$, let $\mathcal G_{M,\alpha}(t)$ denote the set of all
binary classification problems $(P^1,P^2)$ such that $\tv(P^1,P^2) \le t$ and
Condition \ref{cond:orlize} holds.
\end{restatable}
The following concept, first introduced in ~\cite{polyanskiy16}, will be
instrumental to us.
\begin{restatable}[Dobrushin curve]{df}{}
Given a Markov kernel $\omega$ on $\mathcal X$, its total-variational Dobrushin
curve is the function $\mathfrak D_{\omega,M,\alpha}:[0, 1] \rightarrow [0, 1]$
defined by
\begin{eqnarray}
\mathfrak D_{\omega,M,\alpha}(t) := \sup_{(P^1,P^2) \in \mathcal
  G_{M,\alpha}(t)}\tv(P^1 * \omega, P^2 * \omega).
\end{eqnarray}
\label{df:dcurve}
\end{restatable}
Our interest in Dobrushin curves lies in the fact that if the classification
problem $(P^1,P^2)$ satisfies condition \ref{cond:orlize} and $\tv(P^1,P^2) \le
t$,
then
\begin{eqnarray}
  \err_\omega^*(P^1,P^2) \ge \frac{1}{2}(1-\mathfrak D_{\omega,M,\alpha}(t)).
  \label{eq:bridge}
\end{eqnarray}
\begin{wrapfigure}{r}{0.39\textwidth}
  \vspace{-.4cm}
  \centering
  \includegraphics[width=.39\textwidth]{sdpi.png}
  \vspace{-.6cm}  
  \caption{Illustration of Corrollary \ref{corr:gausscurve} for different
    moment contraints on the $P^k$'s. The Bayes-optimal error always strictly
    dominates the standard Bayes-optimal error, by an amount corresponding to
    the shaded areas. For example, the left endpoint of the x-axis
    corresponds to maximally easy standard classification problems
    (Bayes-optimal error = 0, or $t = 1$ in the corrolary). In the presence of
    noise corruption, the noisy Bayes-optimal error is strictly positive.}
 \end{wrapfigure}
This is a direct consequence of Lemma \ref{lm:bayesoptomega}.
%  \vspace{-.5cmcm}
% In the above definitions, we have dropped the dependence on $\alpha$ and $M$
% for simplicity of notation.
The following theorem is one of our main results. It follows the line
of ~\cite[Theorem 4]{polyanskiy16}, which was proposed in the
context of information transmission across additive noise channels. Our
generalization is two-fold. First we consider general Markov kernels on general
metric spaces, in place of additive noise channels in some $\mathbb R^m$.
Second, we work in general abstract metric spaces instead of finite-dimensional
euclidean spaces.
\begin{restatable}[Strong DPIs from moment / tail bounds]{thm}{kingkong}
Let $\omega$ be a Markov kernel on  $\mathcal X$ and let $\theta:[0,\infty)
\rightarrow [0, 1]$
be a
% concave
% non-decreasing
function such that Condition
\ref{cond:lips} holds. Define the function $\bar{\theta}:[0,\infty) \rightarrow
[0, 1]$ by $\bar{\theta}(r) = \sup_{0 \le s \le r}\theta(s)$ and let
$\bar{\theta}^{cc}$ be the concave envelope (i.e smallest concave majorant) of
$\bar{\theta}$. Then for every $t\in (0, 1]$ and classification problem
$(P^1,P^2) \in \mathcal G_{M,\alpha}(t)$, we have
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{itemize}                                                               %
%   \item {\bfseries Bounds on Dobrushin curve.} We have                        %
% \begin{eqnarray}                                                              %
% \mathfrak D_{\omega,M,\alpha}(t) \le                                          %
%   t\bar{\theta}^{cc}(2M^{-1}(\alpha/t)+d(\mu_1,\mu_2)).                       %
%   \label{eq:oneside}                                                          %
% \end{eqnarray}                                                                %
% Moreover, if the inequality in Condition \ref{cond:lips} is an equality, then %
% the bound in \eqref{eq:oneside} is tight, i.e                                 %
% \begin{eqnarray}                                                              %
%  \mathfrak D_{\omega,M,\alpha}(t) \ge t\bar{\theta}(2M^{-1}(\alpha /t)).      %
% \label{eq:otherside}                                                          %
% \end{eqnarray}                                                                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \item {\bfseries Bounds on noisy Bayes-optimal error.} We have
  \begin{eqnarray}
  \err^*_\omega(P^1,P^2) \ge
    \frac{1}{2}\left(1-t\bar{\theta}^{cc}(2M^{-1}(\alpha/t) +
    \Delta)\right),
    \label{eq:noisyrisk}
  \end{eqnarray}
  where $\Delta := d(\mu_1,\mu_2)$.
% \end{itemize}
\label{thm:kingkong}
\end{restatable}
% \begin{proof}
%  See Appendix.
% \end{proof}
% % \vspace{-.5cm}
The above theorem gives precise control on the increase in hardness of
statistically testing between $P^1$ and $P^2$, as a function of the noise and
moment constraints on the $P^k$'s.
\input{gausscurve.tex}

\subsection{Optimal low-dimensional adversarial noise model from covariance
  structure of data}
We now show how to exploit the covariance structure of the features to engineer
a multivariate Gaussian noise kernel which will do the most damage to Bayes-optimal error.

Let $\Sigma$ be an $m$-by-$m$ positive semi-definite matrix and consider the
(possibly degenerate ) elliptic Gaussian noise kernel $\omega^\Sigma$ on
$\mathbb R^m$ given by $\omega^\Sigma_x = \mathcal N(x,\Sigma)$ for all $x \in
\mathbb R^m$. The matrix $\Sigma$ indices a pseudo-metric $\mathbb R^m$ (usually
referred to as \emph{Manahalobis ``distance''}), given by $d_\Sigma(x,x') :=
\|x-x'\|_{\Sigma^\dagger} = \sqrt{(x-x')^T\Sigma^\dagger(x-x')}$, for all $x,x'
\in \mathbb R^m$. Our interest in this pseudo-metric lies in the fact that
$\tv(\omega^\Sigma_x,\omega^\Sigma_{x'}) = \theta(d_\Sigma(x,x'))$, where
$\theta:[0,\infty) \rightarrow [0, 1)$ is the increasing function defined by
$\theta(r)=2\Phi(r/2)-1$, and $\Phi$ is CDF of the standard normal distribution.
This is a direct consequence of formula \eqref{eq:tvgauss}.
Now, consider the quadratic moment function $M(r) := r^2$. Let $\Sigma_k$ and
$\mu_k$ bet the covariance matrix and mean of the features $X$ conditioned on
$Y=k$, and set $\Sigma_0 := (\Sigma_1+\Sigma_2)/2$. Note that positive
semi-definite matrix $\Sigma_0$ is the unconditional covariance matrix of the
features. Then, one computes
\begin{eqnarray*}
  \begin{split}
\mathbb E_{x \sim P^k}M(d_\Sigma(x,\mu_k)) &= \mathbb E_{x \sim
  P^1}\|x-\mu_k\|_{\Sigma^\dagger}^2 = \trace(\Sigma^\dagger\Sigma_k).
\end{split}
\end{eqnarray*}
Thus
$
\mathbb E_{x \sim P^1}M(d_\Sigma(x,x_0)) + \mathbb E_{x \sim
  P^2}M(d_\Sigma(x,x_0)) = \trace(\Sigma^\dagger(\Sigma_1+\Sigma_2)) = 2\alpha(\Sigma),
$
where
\begin{eqnarray}
  \alpha(\Sigma) := \trace(\Sigma^\dagger \Sigma_0).
\end{eqnarray}
Therefore, for each potential covariance matrix $\Sigma$ for the adversarial
noise distribution, the classification problem $(P^1,P^2)$ satisfies Condition
\ref{cond:orlize} for the $d=d_\Sigma$ and $\alpha=\alpha(\Sigma)$.

Note that if $z \sim \omega_x^\Sigma$, then $\mathbb E\|z-x\|^2 = \trace\Sigma$.
The idea is then to construct a noise covariance matrix $\Sigma$, under a power
constraint $\trace\Sigma \le s$ for $s > 0$, which recks the classification problem $(P^1,P^2)$
as much as possible. To this end, let $(\lambda_1,\ldots,\lambda_m)$
be the vector eigenvalues of $\Sigma_0^{1/2}$ (i.e the positive square-roots of
the eigenvalues of $\Sigma_0$), and set $s := m\sigma_0^2$, with $\sigma_0 > 0$.
\begin{restatable}{lm}{stablerank}
  Let $\Sigma_0=U\diag(\sigma^2_1,\ldots,\sigma_m^2)U^T$ be the SVD of the
  unconditional covariance matrix $\Sigma_0$ with $\sigma_1^2 \ge \ldots \ge
  \sigma_m^2 \ge 0$. Subject to the constraints $\Sigma \succeq 0$, $\rank\Sigma
  \le r$, and $\trace \Sigma \le m\sigma_0^2$, the minimal value of
  $\alpha(\Sigma)$ is $\alpha^* =
  (\sum_{j=1}^r\sqrt{\sigma_j^2})^2/(m\sigma_0^2)$, and this value is attained
  at $\Sigma = \widetilde{\Sigma}$, where
  \begin{eqnarray}
    \widetilde{\Sigma} = % \dfrac{s}{\trace C^{1/2}}C^{1/2} =
    \dfrac{m\sigma_0^2}{\sum_{j=1}^r\sqrt{\sigma_j^2}}U\diag(\sqrt{\sigma_1^2},
    \ldots, \sqrt{\sigma_r^2})U^T.
  \end{eqnarray}
  Moreover, we have the upper-bounds
  $\alpha^* \le
\dfrac{1}{\sigma_0^2}\left(\dfrac{\sum_{j=1}^r\sqrt{\lambda^2_j}}{\sqrt{m}}\right)^2
\le \dfrac{1}{\sigma_0^2}\left(\dfrac{r\sqrt{\|\Sigma_0\|_{op}}}{\sqrt{m}}\right)^2$,
where $\lambda_1^2 \ge \ldots \ge \lambda_m^2 \ge 0$ are the eigenvalues of
$\Sigma_0$ and  $\|\Sigma\|_{op} = \lambda_1^2$ is its spectral / operator norm.
\label{lm:man}
\end{restatable}

This leads us to the following theorem, which is one of our main results.
\begin{restatable}[Optimal low-dimensional adversarial noise]{thm}{}
Consider a classification problem $(P^1,P^2)$ on $\mathbb R^m$ with finite
covariance matrices and zero means (i.e the problem is centered)
and let $\tv(P^1,P^2) \le t$. Let $r \in \{1,\ldots,m\}$ and take
$\widetilde{\Sigma} \in \mathbb R^{m \times m}$ and $\sigma_0>0$ as in Lemma
\ref{lm:man}. Then, the noisy Bayes-optimal error for the classification problem
$(P^1,P^2)$ under corruption from the elliptic Gaussian noise kernel
$\omega^{\widetilde{\Sigma}}$ satisfies
\begin{eqnarray}
  \err^*_{\omega^{\widetilde{\Sigma}}}(P^1,P^2) \ge
  \frac{1}{2}\left(1-t\left(2\Phi\left(\frac{\sigma/\sqrt{t}+\Delta/\sqrt{m}}{\sigma_0}
  \right)-1\right)\right),
\end{eqnarray}
where $\Delta := \|\mu_1-\mu_2\|$ and
$\sigma:=\sum_{j=1}^r\sqrt{\lambda_j^2}/\sqrt{m} \le
(r/\sqrt{m})\sqrt{\|\Sigma_0\|_{op}}$.
\end{restatable}

\begin{proof}
  Follows from Lemma \ref{lm:man} and Thm. \ref{corr:gausscurve} with
  the quadratic moment function $M(r) := r^2$.
\end{proof}

The constant $\sigma > 0$ the theorem has an geometric
interpretation: it is a measure of the ``effective'' sparsity of the
spectrum of the unconditional covariance matrix $\Sigma_0$ of the features
%,since one easy verifies that $\eta \le \card(\{1 \le j \le m \mid \lambda_j \ne
% 0\})$.
One the other hand, $\theta$ is a measure of the signal-to-noise ratio in
the classification problem.

==> supp_preamble.tex <==
All through this supplemental and the main manuscript, $\mathcal X$ denotes the feature space.
% At times, this will be a metric space with metric denoted $d_{\mathcal X}$ or $d$ for short.
% The space of labels is $\mathcal Y = \{1,2\}$. There is a
The \emph{label (aka classification target)} is a random variable $Y$ with
values in $\mathcal Y = \{1,2\}$, and random variable $X$ called the
\textit{features}, with values in $\mathcal X$. We only consider binary
classification problems in this work. The goal is to predict $Y$ given $X$. This
corresponds to prescribing a measurable function $h:\mathcal X \rightarrow
\{1,2\}$, called a \emph{classifier}. Let $P$ be the (unknown) joint probability
distribution of $(X,Y)$. The goal of learning is to find a classifier $h$, such
that $h(X) = Y$ as often as possible, possibly under additional constraints.
% The presentation of more notation is deferred to section \ref{sec:bayesian} when we will have a genuine need for it.

\begin{mdframed}
{\bfseries General framework.} In this work, as in ~\cite{bhagoji2019}, we will
only consider binary classification problems under adversarial attacks, where
the labels are equiprobably , i.e $\mathbb P(Y=1)=\mathbb P(Y=2)=1/2$. These
assumptions are technical requirement needed to apply the Kantorovich-Rubinstein
duality formula of optimal-transport. Multiclass problems can be considered in one-versus-all fashion.
We will denote $P^k := \frac{1}{2}\mathbb P(X|Y=k)$ for $k=1,2$, so that the
classification problem is entirely captured by the pair $P=(P^1,P^2)$, called a
\emph{binary experiment}.
\end{mdframed}

\paragraph{Total-variation.} $\tv(Q,Q')$ denotes the total-variation distance between finite measures $Q$ and
$Q'$ on the same measurable space (typically the feature space , $\mathcal X$).

\input{adversarial_notations}
\input{transport.tex}


==> transport.tex <==
\subsection{A premier on optimal transport theory}
The theory of optimal transportaton will be central in our study of adversarial
attacks. The reader should see ~\cite{Villani} for a detailed exposition on
optimal transport theory. We recall the key notions here. Given $p \in
[1,\infty)$ and a distance $d:\mathcal X^2 \rightarrow [0,\infty)$, $\mathcal
W_d$ will denote the $p$-Wasserstein space of Radon measures $\mu$ on $\mathcal
X$ such that $\int_{\mathcal X}d(x,x_0)^p\diff\mu(x) < \infty$ for some (and
therefore, for all!) $x_0 \in \mathcal X$. Given $\mu,\nu \in \mathcal W_{d,p}$,
the quantity
\begin{eqnarray}
W_{d,p}(\mu,\nu) := (\inf_{\pi \in \Pi(\mu,\nu)}\mathbb E[d(X_1,X_2)^p])^{1/p}
\label{eq:wass}
\end{eqnarray}
is the Wasserstein distance between $\mu$ and $\nu$, $\Pi(\mu,\nu)$ denotes the
set of all couplings of $\mu$ and $\nu$, i.e all measures $\pi$ on $\mathcal
X^2$ with marginals $\mu$ and $\nu$ respectively, and the random pair $(X_1,X_2)$
is distributed according to $\pi$, written $(X_1,X_2) \sim \pi$. We shall usually
consider more general (non-metric) cost functions, $c:\mathcal X^2 \rightarrow
[0, \infty)$ which are only assumed to be measurable, and still write $\mathcal
W_c$ to denote the RHS of \eqref{eq:wass}. Note that if $c$ is just
lower-semicontinuous, then $W_c$ is still a distance on the $\mathcal W_c$.


==> uap.tex <==
\section{On the existence of transferable universal adversarial perturbations}
\label{sec:uap}
In this section, we will be concerned with classification problems on $\mathbb
R^m$, where the dimension $m$ is ``large''. As in section
\ref{subsec:notations}, let $P_{XY}$ be the (unknown) joint distribution of the
feature vector $X$ and the label $Y$. Recall notations from the previous
section, where we succinctly refer to the problem by the pair $(P^1,P^2)$, where
$P^k$'s are the unnormalized class-conditional distributions defined in
\eqref{eq:pk}.

\subsection{Preliminaries}
Given a classifier $h:\mathcal X \to \{1,2\}$, a universal adversarial
perturbation (UAP) is a fixed vector $v \in \mathbb R^m$ which fools $h$ on a
proportion of the input samples, i.e
$$
\fr(h; P^1, P^2) := \sum_{k=1}^2P^k(\{x \in \mathbb
R^m \mid h(x\pm v) \ne k\}) = P_{X,Y}(h(X \pm v) \ne Y) \ge \Delta_h > 0,
$$
$\fr(h; P^1, P^2)$ is called the \emph{fooling rate} of $v$ on the classifier
$h$. Of course, such a perturbation is only genuine if its norms $\|v\|$ is
``small'' compared to the norm of a typical feature vector. The seminar work
~\cite{unipert} empirically showed that deep neural nets admit universal
adversarial perturbations with nonzero success rates. In a follow-up paper
~\cite{moosavi17}, the same authors proved the existence of universal
adversarial perturbations gauranteed if the decision boundary of the classifier
is nonnegatively curved almost every where in the feature space. In contrast, we
will make assumptions not on the classifiers, but on the class-conditional
distributions.

\begin{restatable}{rmk}{}
  Our notion of ``fooling'' is stronger than that used in the literature. Indeed,
  ~\cite{moosavi17,unipert} counts / measures the proportion of inputs $X$ for
  which which $h(X\pm v) \ne h(X)$, while we measure the proportion of inputs
  $h(X\pm v) \ne Y$, where $Y$ is the true label of $X$. Of course, the two notions
  are equivalent if the classifier $h$ is perfect (i.e has zero classification
  error), but in general they are different.
\end{restatable}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{restatable}{df}{}                                                                %
%   A transferable universal adversarial perturbation (UAP) is a fixed vector $v \in      %
% \mathbb R^m$ which will fool \emph{any} classifier on a fraction of the input data, i.e %
% $$                                                                                      %
% \fr^*_v(P^1,P^2) := % \inf_{h}P_{X,Y}(h(X \pm v) \ne Y) =                               %
% \inf_{h}\fr_v(h;P^1,P^2) \ge \Delta,                                                    %
% $$                                                                                      %
% for some $\Delta \in (0, 1]$. The largest such $\Delta$ is called the                   %
% \emph{fooling rate} of the vector $v$.                                                  %
% \end{restatable}                                                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Our goal is to show that under moment conditions
\ref{cond:orlize} on the class-conditional distribution, introduced in the
previous section, for a classification problem on $\mathbb R^m$, there exists a
positive constant $\Delta$ such that every classifier admist a UAP
with $\ell_2$-norm $\mathcal O(\sqrt{m})$ with fooling rate at least $\Delta$.

\subsection{Main result: existence of universal adversarial perturbations}
Consider a classification problem $(P^1,P^2)$ on $\mathbb R^m$. Let $t
\in [0, 1]$ and suppose $(P^1,P^2) \in \mathcal G_{M,\alpha}(t)$. Finally, let
$h:\mathcal X \to \{1,2\}$ be any classifier. The following is the main result
of this section, and one of tha main contributions of our manuscript.
\begin{restatable}[Existence of UAPs of size $\mathcal O(\sqrt{m})$]{thm}{tuap}
  For every $c > 0$, the there exists a fixed vector $v \in \mathbb R^m$ with
  $\|v\| \le c\sqrt{m}$, with fooling rate
  \begin{eqnarray}
\fr_v(h; P^1,P^2) \ge
\frac{1}{2}\left(1-
  t\left(2\Phi\left(\frac{M^{-1}(\alpha/t)}{c}\right)-1\right)\right)
    % - \frac{0.4t}{m}.
    + \mathcal O\left( \frac{1}{m} \right),
    \label{eq:tuap}
  \end{eqnarray}
  where $\Phi$ is the standard normal CDF.
  \label{thm:tuap}
\end{restatable}
Actually, we will prove a stronger result, namely: if
$u$ is drawn uniformly at random from the origin-centered ball of radius
$c\sqrt{m}$ in $\mathbb R^m$, then
\begin{eqnarray}
%  \inf_{(P^1,P^2) \in \mathcal G_{M,\alpha}(t)}
  \mathbb E_u [\fr_u(h; P^1, P^2)] \ge
\frac{1}{2}\left(1-
  t\left(2\Phi\left(\frac{M^{-1}(\alpha/t)}{c}\right)-1\right)\right)
  + \mathcal O\left( \frac{1}{m} \right).
  \label{eq:uniform}
\end{eqnarray}  
\begin{proof}[Proof of Thm. \ref{thm:tuap}]
  Recall notation and terminology from section \ref{subsec:markov}.
  We start by reducing our situation to  a problem of corruption by random
  noise. Indeed, for $ x \in \mathbb R^m$, let $B(x)$ be the ball of radius
  $c\sqrt{m}$ and center $x$. Let $\omega^{\unif}$ be the Markov kernel with
  transition probabilities defined for every $x \in \mathbb R^m$, by
  $\omega_x^{\unif} = \unif(B(x))$, the uniform distribution on $B(x)$.
  Equivalently, $\omega_x^{\unif}$ is the translation by $x$, of the uniform
  distribution on $B(0)$. Let $u \sim \unif(B(0))$. One computes
  \begin{eqnarray}
    \begin{split}
  \sup_{\|v\| \le c\sqrt{m}} \fr_v(h; P^1,P^2) &\ge \mathbb E_u \fr_u(h;
  P^1, P^2)
  =: \mathbb E_u\sum_{k=1}^2P^k(\{x \mid h(x \pm u) \ne
  k\})\\
  & \ge \sum_{i=1}^2(P^k * \omega^{\unif})(\{x \mid h(x) \ne k\})
  =: \err_{\omega^{\unif}}(h; P^1,P^2)\\
  &\ge \err^*_{\omega^{\unif}}(h; P^1,P^2),
\end{split}
    \label{eq:reduction}
  \end{eqnarray}
where $\err^*_{\omega^{\unif}}(P^1,P^2)$ is the noisy Bayes-optimal error for
the classification problem $(P^1,P^2)$, under random corruptions as prescribed
by the Markov kernel $\omega^{\unif}$. It thus remains to lower-bound
$\err^*_{\omega^{\unif}}(P^1,P^2)$.

Now, by standard arguments in high-dimensional geometry, if $z_1 \sim \mathcal
N(0, c^2)$, then each coordinate $u_j$ of $u$ is distributionally equal to
$z_1$, and the approximation error in Kolmogorov distance\footnote{The
  Kolmogorov distance between two probability distribution
  functions $F_1$ and $F_2$ on $\mathbb R$ is defined by $K(F_1,F_2) :=
  \|F_1-F_2\|_\infty := \sup_{x \in \mathbb R}|F_1(x)-F_2(x)$.} is at most
$1/(2m)$. Thus,
  \begin{eqnarray*}
    \begin{split}
  \tv(\omega^{\unif}_x, \omega^{\unif}_{x'}) &= 1 - \frac{\vol(B(x) \cap B(x'))}{
  \vol(B(x))} = 1 - \frac{\vol(B(0) \cap B(x'-x))}{
  \vol(B(0))}\\
&= 1 - \mathbb P(|u_1| \ge \|x'-x\|/2)
=\mathbb P(|z_1| \le \|x'-x\|/2) + \mathcal O(1/m)\\
& = \theta(\|x'-x\|) + \mathcal O(1/m),
\end{split}
  \end{eqnarray*}
  where $\theta(r):= \mathbb P(|z_1| \le r) =
  2\Phi(r/(2c)) - 1$ for all $r \ge 0$. Thus, our situation is reduced to that Corollary
  \ref{corr:gausscurve} with $\varepsilon=c$, and we get
  $$
\err^*_{\omega^{\unif}}(P^1,P^2) = \frac{1}{2}\left(1-
  t\left(2\Phi\left(\frac{M^{-1}(\alpha/t)}{c}\right)-1\right)\right)
  + \mathcal O\left( \frac{1}{m} \right).
  \label{eq:uniform}
  $$
  Combining with \eqref{eq:reduction} then completes the proof.
\end{proof}

\subsection{Interpreting Theorem \ref{thm:tuap}}
\begin{figure}[!htbp]
    \begin{minipage}{0.5\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{sdpi.png}
  \end{minipage}
  \begin{minipage}{0.5\textwidth}  
    \caption{Graphical illustration of Thm. \ref{thm:tuap}. The left end of
      the x-axis corresponds to ``easy'' classification problems, while the
      right end corresponds to ``hard'' classification problems. The diagonal
      corresponds to the classical Bayes-optimal error rate without any attack. The
      different colored regions correspond to the fooling rates
      of universal adversarial perturbations (UAP) $v \in \mathbb
      R^m$ with $\|v\| \le \sqrt{m}$, and for different moment conditions on the
      class-conditional distributions. The upper boundaries of the regions
      correspond to the RHS of inequality \eqref{eq:tuap}.}
    \end{minipage}
   \label{fig:dob}
 \end{figure}
 Figure \ref{fig:dob} is a graphical illustration of the result.
 The left end of the x-axis corresponds to ``easy'' classification problems, while the
 right end corresponds to ``hard'' classification problems. 
Recall, as in the end of section
\ref{subsec:adv_notations}, that in classical machine learning (i.e clean, aka
without any attack), the Bayes-optimal error is exactly
$\frac{1}{2}(1-\tv(P^1,P^2))$. If the classification problem is subject to
adversarial attacks, one would expect the Bayes-optimal error to increase as a
function of the attack budget (the signal received by the classifier is
compromised). It has been empirically observed ~\cite{moosavi17} for most
problems in computer vision (classification of images), one can add a carefully
crafted (i.e optimized) perturbation vector to an image and change the
prediction of the classifier (e.g deep neural network). It has also been
observed that these so universal adversarial perturbations, once optimized for a
deep neural network, can be successfully used to fool other deep neural networks
on the same problem ~\cite{moosavi17}. Our Thm. \ref{thm:tuap}
Thm. \ref{thm:tuap} formally proves the existence of transferable UAPs with
nonzero misclassification rate, under moment conditions \ref{cond:orlize} on the
The result is universal in the sense that it does not depend on the specific
properties of any classifier; it applies uniformly on all classifiers.


